IPFormer-VideoLLM: Enhancing Multi-modal Video Understanding for Multi-shot Scenes

Video Large Language Models (VideoLLMs) have demonstrated remarkable understanding capabilities, but are found struggling to tackle multi-shot scenarios,e.g., video clips with varying camera angles or scene changes. This challenge can render failures such as instance identity forgetting and key frame negligence. In this work, we first attribute the challenge to the lack of multi-shot annotations among existing datasets and therefore we introduce a new dataset termed MultiClip-Bench, featuring dense descriptions and instruction-based question-answering pairs tailored for multi-shot scenarios. We empirically find that the training set significantly boosts the multi-shot performance, while the testing benchmark provides a reliable measure of the model capability in multi-shot scenarios. By further analyzing and discovering that current models only encode instance features in a discrete or lossy manner, at the risk of missing identity information, we then contribute a new model IPFormer-VideoLLM. Its key idea is the injection of instance-level features as instance prompts through an efficient attention-based connector. This allows for the aggregation of instance-specific information across scenes. Experiments demonstrate that our proposed dataset and model not only enhance the multi-scene video understanding significantly, but also offer distinct advantages across various video benchmarks.

==> ICCV2025-Author-Kit-Feb/preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> ICCV2025-Author-Kit-Feb/sec/0_abstract.tex <==
\begin{abstract}

Video Large Language Models (VideoLLMs) have demonstrated remarkable understanding capabilities, but are found struggling to % handle
tackle multi-shot scenarios, \textit{e.g.}, video clips with varying camera angles or scene changes. % The multi-shot challenge tends to cause failures like 
This challenge can render failures such as instance identity forgetting and key frame negligence. In this work, we first attribute the challenge to the lack of multi-shot annotations among existing datasets and therefore we introduce a new dataset termed \textbf{MultiClip-Bench}, featuring dense descriptions and instruction-based question-answering pairs tailored for multi-shot scenarios. We empirically find that the training set significantly boosts the multi-shot performance, while the testing benchmark provides a reliable measure of % reasonably reflects 
the model % power
capability in multi-shot scenarios. % against the multi-shot challenge. 
% For a second model-level contribution, we 
By further analyzing and discovering that current models only encode instance features in a discrete or lossy manner, at the risk of missing identity information, we then contribute a new model % As a remedy, we introduce 
\textbf{IPFormer-VideoLLM}. % which 
Its key idea is the injection of instance-level features as instance prompts through an efficient attention-based connector. This allows for the aggregation of instance-specific information across scenes. Experiments demonstrate that our proposed dataset and model not only enhance the multi-scene video understanding significantly, but also offer distinct advantages across various video benchmarks. The code and model will be available.
\end{abstract}

==> ICCV2025-Author-Kit-Feb/sec/1_intro.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.95\linewidth]{pic/F1_L.pdf}
\caption{\textbf{Multi-shot Transitions} Video-LLaVA uses full projection, while VideoChat2 reduces video tokens via attention mechanisms. In scenes with discontinuous character appearances (multi-scene transitions), existing models often fail to distinguish characters, leading to counting errors. Our method compresses tokens and uses detectors and clustering to generate instance prompts, to guide attention fusion across scenes and enhance accuracy.
}	\label{fig:1}
\vspace{-13pt}
\end{figure}

\section{Introduction}
%The development of large language models (LLMs) [] has paved the way for Multi-modal Large Language Models (MLLMs) [],  and the integration of visual encoders with pre-trained LLMs to form visual multi-modal large models [] has gained significant research attention. 
Large Multi-modal Models (LMMs) ~\cite{alayrac2022flamingo,driess2023palm,huang2023language,li2023blip} built by connecting Large Language Models (LLMs) as the brain with specialized encoders, % as the receptor, 
have yielded remarkable progress in tasks involving multiple modalities.
% across image~\cite{liu2023visual,liu2024improved,chen2024expanding,alayrac2022flamingo}, video~\cite{li2023videochat,li2024mvbench,liu2024mmbench}, audio~\cite{chu2023qwen,rubenstein2023audiopalm}, etc. 
In the domain of video,
recent Video Large Language Models (VideoLLMs)~\cite{li2023videochat,li2024mvbench,liu2024mmbench,bai2025qwen2,li2024llava,wang2022internvideo} % can understand text and video with the integretion of LMMs, enabling more efficient video understanding and interaction. And there are multiple works designing 
have customized domain-specific model architectures~\cite{team2024gemini,li2023videochat,cheng2024videollama,qu2024ts} and datasets/benchmarks~\cite{maaz2024videogpt+,krishna2017dense,wang2023internvid}, 
% promote the development of addressing tough 
significantly advancing many video understanding problems such as long video understanding~\cite{liu2024st,song2024moviechat}, fine-grained understanding~\cite{wang2022internvideo,li2024llava}, and temporal localization~\cite{chen2024timemarker,wang2024grounded,patraucean2023perception,li2023seed}. 

Although current VideoLLMs perform % effectively and robust 
well in % simple
most scenarios, % we find that 
they exhibit notable deficiencies in multi-shot scenes, \textit{e.g.}, % the model is given 
video clips captured from various angles of view or different scenes. Compared to single-shot videos, multi-shot ones involve more visual clues and more % complicated
complex object relationships, requiring % great
advanced information extraction and instance-level comprehension capabilities. Fig.~\ref{fig:1} illustrates a failure case in a multi-shot scenario. Given % several 
video clips from different cameras depicting % one
the same talent show, the models are asked to count the number of people who have ever appeared. Surprisingly, for this seemingly simple question, Video-LLaVA~\cite{lin2023video} and VideoChat2~\cite{li2024mvbench} answered $2$ and $4$ respectively, while the ground truth is $3$. 

Why do existing VideoLLMs fail in such an easy case? We attribute the failure to two % key points
key factors: data and model limitations. First, an examination of commonly used datasets reveals a scarcity of training data for multi-shot scenarios. Current annotations % emphasis 
primarily focus on single-shot videos, with monotonous camera changes, slow object movement, and few scene transitions. In contrast, the descriptive quality of high-dynamic multi-shot videos remains substandard. Those multi-shot annotations tend to provide only brief overviews of the video, while lacking details and depth. % , while not cover various required details. 
Moreover, on the test end, the widely used benchmarks \cite{wang2023internvid,krishna2017dense,maaz2024videogpt+,li2024mvbench,fu2024video} can hardly reflect the ability for multi-shot video understanding due to the absence of relevant test cases. % in their design. 
% Therefore, it is urgent to propose a tailored training set and benchmark for multi-shot video understanding.

To fill this gap, we first introduce a multimodal video understanding benchmark called \textbf{MultiClip-Bench}. The creation of MultiClip-Bench involves both video annotation and question-answer (QA) formulation. For annotation, we segment the video into key frames, annotate each key frame with character IDs, and label the video with dense captions and character information.
% Compared to existing benchmarks, our dataset stands out in its annotation format and question design. 
% Ours video descriptions are built with three key elements: keyframe annotations with character IDs, dense captions, and character information annotations, all aimed at covering multi-scene understanding.
% We segment the video into keyframes and annotate each keyframe sequence with character IDs to ensure correct association of individuals across scenes, maintaining character consistency. Then, we label the video with dense captions and character information.
% , which also connect fragmented scenes involving the same person.
In the design of QA pairs, we also focus on the challenges of multi-shot scenarios, particularly on cases where characters appear discontinuously across multiple scenes or have brief appearances, and generate a large number of QA pairs accordingly.
% These efforts address potential issues in multi-shot scenes and generate question-answer pairs to enhance instruction-following capabilities. 
Finally, we manually selected a subset of $2,750$ pairs to constitute the test set, with answers verified, refined, and categorized to form the benchmark.

Although significant improvement is observed when using the MultiClip training set, we found several typical failure cases of current models when handling multi-shot videos. Two significant deficiencies of current VideoLLMs are identified: i) the lack of instance consistency preservation during scene transitions; and ii) the occlusion of information about briefly appearing characters caused by large data volumes in the video. To address these challenges, % with 
we propose a new model, \textbf{IPFormer-VideoLLM}, which utilizes \textit{instance prompts} to guide attention for more effective instance feature preservation. Specifically, we sample and aggregate features from bounding-box regions to form instance features, and inject them as visual prompts into the query to guide attention. Besides significant performance gains, it reduces tokens to less than $10\%$ of the baseline, cuts training time by $75\%$, and boosts inference speed. 
%Experiments show strong performance on our benchmark and others, ith further performance improvements achieved when trained on our proposed dataset.

Experimental results demonstrate that our proposed model performs strongly on both existing benchmarks and our MultiClip-Bench, with further performance improvements observed when utilizing our proposed training dataset. Specifically, compared to the baseline model Video-LLaVA~\cite{lin2023video}, our model achieves a significant improvement of \textcolor{DarkGreen}{\textbf{2.3\%}}  on MultiClip-Bench. With the support of our training dataset, the performance on MultiClip-Bench increases by \textcolor{DarkGreen}{\textbf{8.5\%}}. Noticeable performance gains are also observed on other datasets. For example, datasets such as NExT-QA~\cite{xiao2021next} and IntentQA~\cite{li2023intentqa} exhibit particularly remarkable enhancements. 
% These results indicate that the multi-shot problems we propose are, in fact, widespread across various benchmarks, but previous benchmarks have failed to adequately address or systematically resolve these multi-shot challenges. %By training with our dataset, these issues are effectively alleviated.
This further validates the significant value of our dataset in addressing the common limitations of multi-shot video understanding.
% Experiments demonstrate that our proposed model exhibits strong performance on both our MultiClip-Bench and other video benchmarks, with further improvements observed when trained on our proposed dataset. Specifically, compared to the baseline Video-LLaVA~\cite{lin2023video}, our model achieves a \textcolor{DarkGreen}{\textbf{+2.3}} improvement on the MultiClip-Bench. % with slight gains on other video benchmarks. 
% With the support of our proposed dataset, the performance on the Multi-Bench % can be further
% further increases by \textcolor{DarkGreen}{\textbf{+8.5}}, and substantial improvements are observed on other datasets as well. Some datasets, such as NExT-QA~\cite{xiao2021next} and IntentQA~\cite{li2023intentqa}, show significant enhancement, thanks in part to the presence of numerous multi-scene examples. 

==> ICCV2025-Author-Kit-Feb/sec/1_intro0.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.95\linewidth]{pic/F1_last.pdf}
\caption{\textbf{Multi-shot Transitions} Video-LLaVA uses full projection, while 
 VideoChat1/2 reduce video tokens using attention mechanisms. In scenes with discontinuous character appearances (multi-scene transitions), existing models often struggle to distinguish characters, causing counting errors. Ours compresses tokens and uses detectors and clustering as instance prompts to guide attention information mixing, improving accuracy.
}	\label{fig:1}
\vspace{-13pt}
\end{figure}

\section{Introduction}
%The development of large language models (LLMs) [] has paved the way for Multi-modal Large Language Models (MLLMs) [],  and the integration of visual encoders with pre-trained LLMs to form visual multi-modal large models [] has gained significant research attention. 
The  Multi-modal Large Language Models (MLLMs) ~\cite{alayrac2022flamingo,driess2023palm,huang2023language,li2023blip,li2023videochat,liu2023visual,wang2024qwen2,zhu2023minigpt} attract significant attention. Among these, 
% video large models
video LLMs~\cite{lin2023video,li2024mvbench,zhang2023video,xu2024pllava,team2024gemini} face numerous challenges, such as long video understanding~\cite{liu2024st,song2024moviechat}, fine-grained understanding~\cite{wang2022internvideo,li2024llava}, and temporal localization~\cite{chen2024timemarker,wang2024grounded,patraucean2023perception,li2023seed}. To meet the demands of these specific tasks,  various video benchmarks and model designs have emerged, demonstrating remarkable capabilities. . %The advent of LLMs has significantly improved the ability to automatically annotate video questions ~\cite{maaz2024videogpt+,li2024mvbench},  and a common practice now is to generate question-answer pairs from detailed video descriptions or captions. 
We find that, despite the existence of many benchmarks~\cite{li2024mvbench,fu2024video,caba2015activitynet,xiao2021next,lei2018tvqa,mangalam2023egoschema,yi2019clevrer} for evaluating video models, they still struggle to effectively reflect the performance in common real-world scenarios, such as multi-shot videos with multiple scene transitions.

\wzc{The Multi-modal Large Language Models (MLLMs) have yielded remarkable results. Regarding video data, there has been a significant emergence of Video LLMs dedicated to long video understanding and fine-grained understanding, which have demonstrated remarkable capability. However, we observe that although current video LLMs have demonstrated robust capabilities in video understanding, they exhibit notable deficiencies in multi-scene videos. }

\wzc{Videos containing multiple distinct scenes are formally termed multi-scene video. Compared to single-scene video, such compositions require enhanced temporal segmentation capacity and instance-level comprehension, thereby enabling robust understanding of dynamic transformations and relational dependencies among instances across scenes. As shown in Fig~\ref{fig:1}, previous video LLMs struggle with the question related to multi-shot scenes. Through investigation of this phenomenon, we show that such issue stems from the scarcity of training data tailored to multi-scenes and architectural limitations in prevailing model frameworks. From a data perspective, while existing video datasets demonstrate quantitative abundance, their compositional emphasis predominantly lies in single-scene, with high-dynamic multi-scenes videos constituting merely marginal proportions. Furthermore, current QA formulations inadequately meet multi-scenes understanding requirements. Current QAs are more for the understanding of the whole video and not for the understanding of the different scene levels. Moreover, current widely used benchmark can hardly reflect the ability for multi-scene video understanding because of the lack of consideration of multi-scene, an important video type, in its design. Therefore, it is essential to propose a tailored training set and benchmark for multi-scene video understanding.}

\wzc{To address the gap in multi-scenario benchmarks, we propose a multimodal video understanding benchmark called \textbf{MultiClip-Bench}. Compared to existing benchmarks\cite{wang2023internvid,krishna2017dense,maaz2024videogpt+,li2024mvbench,mangalam2023egoschema,fu2024video}, our dataset stands out in its annotation format and question design. %First, we introduce an automatic selection and annotation pipeline to create the dataset. 
 Ours video descriptions are built on three key elements: keyframe annotations with character IDs, dense captions, and character information annotations, all aimed at covering multi-scene understanding. We segment the video into keyframes and annotate each keyframe sequence with character IDs to ensure correct association of individuals across scenes, maintaining character consistency.  Based on this, we generate dense captions and character information annotations for video, which also connect fragmented scenes involving the same person. We then focus on scenarios where characters appear discontinuously across multiple scenes or have brief appearances (time criteria are used only for dataset generation). These efforts address potential issues in multi-shot scenes and generate question-answer pairs to enhance instruction-following capabilities. From these, we manually selected a subset of $2,750$ pairs to form the test set, with answers verified, refined, and categorized to create the Benchmark.}

 \wzc{Thanks to the benchmark we proposed, we found that existing models perform poorly in handling multi-shot videos. To obtain the ideal model satisfying video LLM,
we identify several requirements for obtaining satisfying video LLM: 
% in the process of obtaining the CAD features, 
(a) efficient processing of large numbers of video frames to preserve key frame information between scene transitions; 
% Second, 
(b) ability to capture information about instances in different scenarios, thus improve cross-scene understanding ability.
Unfortunately, current video LLMs do not satisfy both conditions and tend to ignore the important instance information in multi-scene video. Motivated by the requirements, we propose a new model named \textbf{IPformer-VideoLLM}, which uses \textbf{instance prompts} to guide attention for better instances feature aggregation. Specifically, we sample and aggregate features from bounding box regions into instance features, injecting them as visual prompts into the query to guide attention. This reduces tokens to under 10\% of the baseline, cuts training time by 75\%, and boosts inference speed. Experiments show strong performance on our benchmark and others, ith further performance improvements achieved when trained on our proposed dataset.
}

Multi-shot videos often present challenges in understanding fragmented scenes. For instance, when multiple people appear in discontinuous scenes, the question "How many people in the video?" (as shown in Fig ~\ref{fig:1}). Such questions, which involve multi-scene transitions, have not been adequately addressed or summarized by existing benchmarks. The main cause lies in the lack of high-quality annotations tailored for multi-scene understanding.  Current video descriptions typically\cite{wang2023internvid,krishna2017dense,maaz2024videogpt+,luo2023valley} provide a general summary of the entire video, focusing on  key actions of key 
 individuals, striking content, or the overall atmosphere. However, this annotations is not suitable for multi-shot scenarios. The core challenge lies in how to separate unrelated scenes and connect multiple related yet discrete shots, which should be considered related. For instance, in Fig.~\ref{fig:1}), the female judge appears in only one frame, which should be treated as an independent scene. Meanwhile, the male judge appears in frames 1, 2, and 8. However, current video annotations often focus solely on describing the key actions or appearance of the man, neglecting his association across different shots, and even entirely omitting any mention of the female judge. Can such annotations help the model recognize that the man at the beginning and end is the same person? Will less prominent scenes, like those with the female judge, be ignored? Moreover, question-answer pairs from these inadequate annotations fail to address the core challenges of multi-scene understanding.

 To address the gap in multi-scenario benchmarks, we propose a multimodal video understanding benchmark called \textbf{MultiClip-Bench}. Compared to existing benchmarks\cite{wang2023internvid,krishna2017dense,maaz2024videogpt+,li2024mvbench,mangalam2023egoschema,fu2024video}, our dataset stands out in its annotation format and question design. %First, we introduce an automatic selection and annotation pipeline to create the dataset. 
 Ours video descriptions are built on three key elements: keyframe annotations with character IDs, dense captions, and character information annotations, all aimed at covering multi-scene understanding. We segment the video into keyframes and annotate each keyframe sequence with character IDs to ensure correct association of individuals across scenes, maintaining character consistency.  Based on this, we generate dense captions and character information annotations for video, which also connect fragmented scenes involving the same person. We then focus on scenarios where characters appear discontinuously across multiple scenes or have brief appearances (time criteria are used only for dataset generation). These efforts address potential issues in multi-shot scenes and generate question-answer pairs to enhance instruction-following capabilities. From these, we manually selected a subset of $2,750$ pairs to form the test set, with answers verified, refined, and categorized to create the Benchmark.

 Through the benchmark we proposed, we found that existing models perform poorly in handling multi-shot videos. These models rely on full projection of visual tokens\cite{lin2023video,li2024llava,xu2024pllava,wang2024qwen2}, to achieve good results, but they are slow and support only a limited number of frames, making efficient token compression a key challenge\cite{bai2023qwen,zhang2025llava,zhang2023video,song2024moviechat,ye2024mplug,liu2024st}. For example, Qformer\cite{li2023blip} mixes frame features using learnable query tokens but faces high training difficulty. Hence our first goal is to design a more efficient compression method to accommodate more frames; Existing models split highly correlated regions into independent tokens, fragmenting instances features. Our second goal is to aggregate these features across scenes. To address this, we propose \textbf{IPformer-videoLLM}, which uses \textbf{instance prompts} to guide attention for better  instances feature aggregation. Specifically, we sample and aggregate features from bounding box regions into instance features, injecting them as visual prompts into the query to guide attention. This reduces tokens to under 10\% of the baseline, cuts training time by 75\%, and boosts inference speed. Experiments show strong performance on our benchmark and others, ith further performance improvements achieved when trained on our proposed dataset.
% The development of large language models (LLMs) has laid the foundation for Multi-modal Large Language Mod
% els (MLLMs), with vision-centric models (e.g., GPT-4o, LLaVA, InternVL series) enabling LLMs to understand visual information such as images and videos. The mainstream approach involves encoding images or video sequences and flattening them then aligning them to the textual space via linear projection[]. However, in practical applications, as shown in Figures ~~\ref{{fig:1}} and ~~\ref{fig:PLLava}, tokenization based on fixed-size patches performs poorly in scenarios involving instance consistency understanding and shot transitions. This may be attributed to: (1) conflicts between language models and visual tokenization, where fixed-size tokenization splits correlated regions into independent tokens, leading to issues like individual truncation and overlooked small objects; and (2) insufficient frame sampling, where limited frames (e.g., 8 frames) fail to capture sufficient visual information in complex scenes. To address these challenges, current models[] adopt higher-resolution images and more frames, significantly increasing computational costs, making efficient video token compression a key focus Among the compression schemes, the attention-based approach achieves a higher compression rate compared to methods like average pooling (avg-pooling), significantly reducing the number of tokens. However, the attention module converges more slowly and typically requires more complex training procedures [] and larger amounts of data [] to effectively learn the attention mechanism and the learnable query. Moreover, its performance often falls short of methods like average pooling. One of our goals is to optimize the attention-based approach so that it can achieve better performance than uncompressed methods (full projection) under the same amount of data.

%语言大模型（LLM）的发展为多模态大模型（LMMs）奠定了基础，其中视觉大模型（如GPT-4o、LLaVA、InternVL系列）赋予了LLM对图像和视频等视觉信息的理解能力。目前主流方法通过Vision Transformer（ViT）将图片或视频序列编码后展平，并利用线性投影将其对齐到文本空间[]。然而，在实际应用场景中，如图1和图2所示，基于等大小token化的方案在处理实例不连续或镜头切换的场景时表现不佳。这可能源于以下原因：1.语言模型与视觉token化的特性冲突：语言模型中单词间具有离散性，而图像等大小token化会将强相关区域分割为独立token，导致人物截断等问题，不利于后续推理。小人物等重要细节容易被忽略，进一步影响模型性能。2.视频帧采样不足：当前模型通常仅使用有限帧数（如8帧），难以提供足够的视觉信息，尤其在复杂场景中可能导致关键信息丢失。为了提升效果，当前模型[]倾向于采用更高分辨率的图像和更多的视频帧数，但这显著增加了计算成本，使得视频信息压缩成为研究重点。现有视频压缩方法多样（详见Related Work）。其中基于注意力机制的压缩方案相较于基于平均池化（avg-pooling）等方法，其压缩率更大，能显著减少token数量，然而这个attention模块收敛慢，他们通常需要更复杂的训练流程[]和更多数据[]去更好学习attenion模块和可学习的query，且效果也不如平均池化等方法。我们的目标之一是优化基于attenion的方案，使其在同样数据的情况下达到相比于不压缩（全投影）更好的性能。

% 1. 因为需要更多的信息，所以需要更多的视觉token，但是如果直接使用的话，对于视觉token当中的冗余性就太强了，从而导致性能虽然提升，但是不值得。2. 因此需要token compression的方式，保存更多有效的token，去除冗余的token。3. 两种基本方式，对于视频而言，因为其对于帧率和分辨率的要求，所以需要更高的压缩率。目前基于attention的压缩方式的压缩率高，但是存在有性能和训练的问题，因此我们的模型的目的就是解决这个问题。提升压缩率，同时有更好的性能和训练收敛。

% 我认为模型这边的说法，需要和multi-shot scenes结合一下。

% 在多场景的视频数据环境下，存在的问题。1. 视频数据需要压缩，从而才可以有更好的理解能力。2. 目前的压缩方法，对于多场景的视频数据效果不佳：因为目前很多压缩是pooling这类的方式，可能会将不属于同一个场景的压缩到一起（一般可能直接的类似于pooling的压缩方式会存在有将不同场景直接合并的问题），但是动态的压缩方式，比如attention的方式，目前的性能和训练时存在明显的问题。这样才能支持存在多场景的视频数据的压缩要求。
% 因此从我们的任务的需求出发， 我们需要开发一个易于训练的，性能好的，动态压缩方式（基于attention）

% The development of video understanding is somewhat constrained by the low quality of video-text data. Existing research [] explores various aspects such as high video quality, video localization, and timestamps. Relevant to our work, ....[] points out that existing video-text datasets lack dynamism, with much of the content being describable by a single image, lacking the temporal understanding challenges unique to video scenarios. In contrast, we focus on the comprehension difficulties caused by multi-shot transitions in videos, such as person re-identification, as shown in Figure ~re. This task requires recognizing the same individual across discontinuous appearances, demanding an understanding of continuity. Previous models and datasets have rarely addressed this scenario, and there is a lack of relevant datasets. 

% 还需要把模型和数据集串起来，可能会更好一些。

%视频理解的发展一定程度受制于视频-文本数据的低质量。现有研究[]从不同的角度研究高视频质量，视频定位，时间戳等方向。其中与我们相关的是,...提出[]现有的视频-文本数据集的动态性差，很多内容是一张图片就能描述的，不具有视频场景下独有的时序理解等困难。而我们专注于视频多镜头切换带来的理解困难，比如行人重识别，如图1所示，要求要能识别不连续出现的人是同一个人，这要求具有理解连贯性。之前的模型和数据很少研究此场景，缺乏相关的数据集。  

% 目前视频理解的难点在于对多场景下的理解，这个其中的一个核心原因是在于目前对于多场景数据集的工作的缺失。 之前的工作xxx。因此我们提出这个数据集对于提升多场景理解，从而提升对于视频理解的能力是必要的。

% In this paper, our research objectives are twofold: (iTo explore a more efficient video visual token compression framework that uses fewer tokens to achieve faster and more efficient visual information processing in multi-shot and other complex scenarios, while maintaining or even improving model performance. (ii To construct a dedicated multi-shot scene dataset, as we found that current research on multi-shot scene understanding lacks specialized datasets, which may severely limit the model's ability to comprehend such scenarios.

% 在本文中，我们的研究目标是提升模型对于多场景的视频数据的理解能力。其中具体的可以分为两个方面，1. 从模型结构上，设计了一个模型视觉token压缩器，有利于提升模型对于包含多场景的视频的理解能力。2. 提升了相关的数据集。

%在本文中，我们的研究目标分为两个方面：1.探索更高效的视频视觉token压缩框架采用更少的toke在多镜头场景及其他复杂场景中实现更快、更高效的视觉信息处理，同时保持或提升模型性能。2.构建多镜头场景相关数据集：我们发现，当前关于多镜头场景理解的研究缺乏专门的数据集，这可能严重限制模型在该场景下的理解能力。

% For the first objective, we propose a compression framework based on cross-attention, drawing inspiration from Conditional-DETR and improving learned queries. Specifically: 1.Injecting frame-level information to enhance token order: We sequentially inject the cls-token and global-avg-token of each frame into each query token, providing guidance for subsequent information mixing and preserving token order. 2.External detector for instance supplementation: To address the lack of instance information, we introduce an external detector to identify all potential instances. Features corresponding to each detected bounding box are sampled and aggregated, then injected into the query tokens. This operation is similar to the anchor mechanism in object detection[], guiding the query tokens in their interaction with subsequent video sequence features. Under the same experimental setup[], we reduce tokens from 8×256 to 8×20, achieving a Speedup is approximately 3 times (excluding the external detector). inference speedup and a 1.1 point performance gain on dataset[].


% For the second objective, we constructed a dataset specifically designed for multi-shot scenes, consisting of two parts: Training set: We propose an automatic selection and annotation pipeline to create the dataset, which includes keyframe annotations, dense captions, and character information annotations to improve the quality of multi-shot scene labeling. We focus on scenarios with discontinuous characters across multiple scenes, identifying potential issues in multi-shot scenes and generating QA pairs to enhance instruction-following capabilities. Test set: From the generated QA pairs, we manually select a subset as the test set, where answers are verified, refined, and categorized to form the final evaluation set. We tested our model and other models on this dataset, demonstrating that our model and training set effectively improve the understanding of multi-shot scenes.
%针对第一点，我们提出了一种基于cross-attenion的压缩框架，并参考了Conditional DETR的设计，对learned query进行了改进。具体方法如下：1.注入帧级信息以增强token顺序性：将每帧的cls-token和global-avg-token按顺序注入到每个query token中，为后续的信息混合提供引导，从而保留token排列的顺序性。为了弥补实例信息的缺失。2.外接检测器以补充实例信息：为了弥补实例信息的缺失，我们引入了一个外部检测器，用于检测潜在的所有实例。通过对每个检测框（box）所在区域的特征进行采样和聚合，将这些实例特征注入到query token中。上述操作与目标检测中的给定anchor机制类似，能引导其query token和之后视频序列的特征混合。针对第二点，我们构建了一个专门面向多镜头场景的数据集，包括以下两部分：训练集：我们提出了自动选择和标注的流程来制作数据集，其内容包含关键帧标注，密集字幕，和人物信息标注来提高多镜头场景标注的质量。我们多场景下不连续人物的场景，挖掘多镜头场景中可能存在的问题，生成QA对，提高指令遵循能力。测试集：对生成的QA对，我们人工选择一部分作为测试集，对答案进行饺子且分类，形成测试集，我在我们的模型和其他模型进行测试，表面我们的模型和训练集能有效提高这个多镜头场景的理解能力。


% 除此以外，也在更广泛的视频benchmark上测试了性能，验证了这个问题是视频理解中广泛存在的。

==> ICCV2025-Author-Kit-Feb/sec/2_Rela.tex <==
\section{Related Work}
\label{sec:Related Work}

% In video LLMs, after feature extraction, video tokens are flattened and projected, then concatenated with text and fed into the LLM. This approach is simple and effective but computationally expensive. To reduce costs, two main strategies exist: 1) Adding cross-attention layers in the LLM to fuse visual content, but this often performs poorly due to insufficient mixing[]; 2) Reducing the number of tokens fed into the LLM, a more popular approach that can also be combined with the first strategy[]. Common methods for the second strategy include using CNNs with average pooling[], fast-slow stream merging[], or attention-based compression[]. However, attention-based methods struggle to preserve token order, conflicting with the sequential nature of LLMs, leading to slower convergence and requiring more training data and complex processes[]. Our research aims to address this by accelerating convergence and simplifying training.
\subsection{Video Benchmark}
Video benchmark evaluations can be categorized into comprehensive assessment sets and task-specific assessment sets. Modern frameworks include MMBench~\cite{liu2024mmbench}, Video-MME~\cite{fu2024video}, and MVBench~\cite{li2024mvbench},  among others. Specifically, Video-MME enhances data diversity through domain hierarchies (6 categories, 30 subclasses) and balanced video durations. MVBench provides a comprehensive evaluation by categorizing tasks into 20 types, facilitating holistic assessment. Task-specialized benchmarks target specific capabilities: Perception Test~\cite{patraucean2023perception} evaluates spatiotemporal reasoning, FunQA~\cite{xie2024funqa} tests models with counter-intuitive scenarios, NExT-QA~\cite{xiao2021next} focuses on object interactions, and IntentQA~\cite{li2023intentqa} emphasizes understanding user intent. However, existing benchmarks primarily concentrate on single-shot or simple scene transitions, offering limited comprehension difficulty, and fail to fully address the unique challenges of multi-shot scenes, such as maintaining character consistency across discontinuous scenes, interpreting short-duration segments, and recognizing outlier events.

\subsection{Video Feature Alignment}
In MLLMs, image or video tokens are flattened and projected after feature extraction, and then concatenated with text before being fed into the LLM~\cite{lin2023video,liu2023visual,liu2024improved}. Although this approach is simple and effective, the large number of tokens, especially those from videos, significantly increases computational costs for the LLM. As MLLMs are increasingly deployed in real-time applications~\cite{ren2024timechat,song2024moviechat,bai2025qwen2,huang2024vtimellm}, enhancing inference efficiency and accommodating more frames have become critical research goals, particularly in multi-shot scenarios. Currently, reducing the number of tokens input to the LLM constitutes the primary strategy. Token compression techniques include downsampling through average pooling~\cite{xu2024pllava,bai2025qwen2,li2024llava}, fast-slow stream merging~\cite{xu2024slowfast,qu2024ts}, compressing videos into fixed-length representations using memory techniques~\cite{song2024moviechat}, and attention-based compression via Q-former~\cite{zhang2023video,bai2023qwen,li2023videochat}. However, crucial information can be lost during token compression, particularly in complex multi-shot scenes. To address this issue, we propose an efficient compression scheme specifically tailored for multi-scene applications. Our approach can accommodate a greater number of frames while effectively preserving essential information.







==> ICCV2025-Author-Kit-Feb/sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> ICCV2025-Author-Kit-Feb/sec/3_Dataset.tex <==
\begin{figure*}[!t]
	\centering
	\includegraphics[width=0.92\linewidth]{pic/F3_L.pdf}
\caption{\textbf{Challenges in Multi-shot Scenarios.} In multi-shot scenarios, Dense description capability of PLLaVA  falters. As shown on the left, the system misses some key frames, only recognizing the woman in green while failing to detect the man in yellow. In the example on the right, the system exhibits person confusion, incorrectly attributing the actions of two individuals to a single person.
}
	\label{fig:PLLAVA}
\end{figure*}
\section{MultiClip-Bench}
% wzc
In this section, we first describe the process of filtering multi-shot videos and creating target video descriptions in \ref{3.1}. Next, we will introduce the generation of multi-shot related QA pairs in \ref{3.2}.

% First, we describe the process of screening multiscene videos and creating video descriptions, as shown in Figure \ref{3.1}. Next, Figure \ref{3.2} illustrates the generation of multi-shot-related question-answer pairs, along with examples and their categorization. 

\subsection{Multi-Shot Description Generation}
\label{3.1}
% wzc
Some widely used video LLMs, such as PLLaVA~\cite{xu2024pllava}, claim to possess strong video understanding capabilities. However, in multi-shot videos (Figure \ref{fig:PLLAVA}), previous VideoLLMs exhibit notable drawbacks, struggling to recognize even simple scenes transitions. A major reason is the lack of tailored multi-shot video data. Motivated by this requirement, we propose MultiClip-Bench, the first multi-shot video dataset, containing a training set and a manually verified test set. As shown in Figure~\ref{fig:2}, we design an effective data engine pipeline, which contains video selection and description generation, for automatic data production. We first introduce the video selection part to demonstrate the method of obtaining the target multi-shot videos.

%\wzc
{\noindent\textbf{Video Selection}} Since the multi-shot videos are difficult to distinguish directly and scenes often change with character transitions, we propose using character changes as a proxy. Additionally, We only retain videos up to two minutes in length, focusing on multi-scene content and excluding interference from other issues such as long duration.%we focus on short videos under two minutes as prior works \wzc{(cite any work)} to reduce complexity. 
 We then employ a coarse-to-fine filtering strategy. In the first stage, a filter based on person instances is employed, using OC-SORT~\cite{cao2023observation}  to perform coarse filtering based on person tracking in order to analyze the trajectories of person IDs. Videos with ID transition exceeding 5 occurrences are retained. In the second stage, we establish two key criteria for the strong close-source video LLM Gemini-1.5-Pro-flash~\cite{team2024gemini} to filter videos: i) Person ID switches within the video, which require transitions in person identities; ii) Clear identification, limiting foreground and background characters to balance scene complexity and computational feasibility.

% Some open-source models, such as PLLaVA, claim to possess strong video description capabilities. However, in multi-shot scenarios (Figure \ref{fig:PLLAVA}), PLLaVA demonstrates notable limitations in video description, struggling to recognize even simple character transitions. We attribute this to insufficient relevant training data, as  training on our MultiClip-Bench dataset corrects these errors. Multiclip-Bench builds a multi-shot video dataset by automatically selecting and annotating videos containing multiple shots, as illustrated in Figure \ref{fig:2}. The specific process is as follows:%However, multi-shot situations are common in real life and should be a focus in video understanding research. Therefore, we attempt to annotate a multi-shot dataset, we address this by automatically selecting and annotating a dataset with videos containing multiple shots, Per Figure\ref{fig:2}.

% \noindent\textbf{Video Selection} 
% We employ a two-stage filtering strategy to filter video data, focusing on short videos under two minutes to reduce complexity. Given the human-centric nature of current visual tasks (e.g., ReID~\cite{ye2021deep,zheng2016person}, behavior analysis~\cite{zhao2017temporal,jhuang2013towards,liu2024end}), we propose dynamic person distribution criteria that retain videos with multi-person interactions and identity switches while discarding scenes with single or static person IDs. In the first stage, coarse filtering based on person tracking~\cite{andriluka2008people,tang2017multiple,mckenna2000tracking} is performed using OC-SORT~\cite{cao2023observation} to analyze person ID trajectories, prioritizing samples with ID switching frequencies above a threshold. In the second stage, refined filtering using Gemini-1.5-Pro-flash~\cite{team2024gemini} ensures selected videos meet three key criteria: (i) Person ID Switching within the video, requiring transitions in person identities; (ii) Person Density Control, limiting visible persons to 2–16 to balance scene complexity and computational feasibility; and (iii) Background Purity, excluding videos with complex background noise (e.g., dense crowds) that could hinder accurate person identification.
\begin{figure*}
	\centering
	\includegraphics[width=0.9\linewidth]{pic/F4_L.pdf}
\caption{\textbf{Description Annotations of MultiClip-Bench} First, we filter the target videos, and then use close-source large video models to generate the three key elements of video description: \textbf{keyframe description}, \textbf{character information}, and \textbf{dense caption}. 
	}
	\label{fig:2}
\end{figure*}

%\wzc
\noindent\textbf{Video Description Generation} Once the target videos are selected, the next step is to obtain descriptions. However, the widely used dense descriptions cannot meet the requirement of multi-shot videos because they often fail to capture character associations across scenes and tend to overlook short or non-critical segments. To address this, we introduce two new annotations: \textbf{keyframe descriptions} with person IDs and \textbf{character information}, which respectively emphasizing the consistency of characters and their features and actions. %which emphasize the consistency and features of characters separately. 
To obtain additional annotations, we propose an automated framework. As shown in Figure \ref{fig:2}, we first select keyframes using PySceneDetect and then use LLaVA-1.5\cite{liu2024improved} to generate detailed description for the selected keyframes, serving as the initial keyframe description. Then we further leverage Gemini to refine the initial keyframe description with the original video, utilizing its strong ability to detect person ID changes and behavioral shifts (see Supplementary Materials for details). By combining the refined keyframe description and the original video, we ultimately produce the dense caption and character information using Gemini. Thus, we obtain the video description, which encompasses three key elements: keyframe description, character information, and dense captions.

% \noindent\textbf{Video Description Generation}
% Complex human interactions in multi-shot scenarios challenge existing dense captioning methods, which often fail to capture character associations across scenes and overlook short or non-critical segments.  To address this, we introduce two new annotations: \textbf{keyframe descriptions} with person IDs and \textbf{character information}. Adding person IDs to keyframe annotations enables consistent tracking across scenes, improving video understanding and aiding tasks like ReID and action recognition. Keyframe-based descriptions also reduce ignored segments. Character information, such as appearance and action sequences, enhances consistent individual understanding.The operations are shown in Figure \ref{fig:2}, we first select keyframes using optical flow changes and use LLava-1.5 \cite{liu2024improved} to generate detailed descriptions for individual frames as the initial keyframe descriptions. However, due to suboptimal optical flow segmentation, we further leverage Gemini for refinement, taking advantage of its strong ability to detect person ID changes and behavioral shifts (see Supplementary Materials for details). By combining the initial keyframe descriptions with the original video, we produce refined keyframe descriptions. These keyframes, along with the original video, are then processed using Gemini to generate character information and dense captions. Thus, our description of a video includes three key elements: keyframe descriptions, character information and dense captions.

Our video data %content %dataset
% integrates data
comes from multiple sources, including Kinetics-710 \cite{li2022uniformerv2}, VideoChatGPT \cite{maaz2023video}, VideoChat \cite{li2023videochat}, YouCook2 \cite{li2023videochat}, NExTQA \cite{xiao2021next}, WebVid \cite{yang2021just,bain2021frozen}, and EgoQA \cite{grauman2022ego4d}. After filtering and annotation, each video contains the three elements as shown in Figure \ref{fig:2}, resulting in a descriptive dataset with 23k high-quality video-text pairs (6.7k videos) tailored for multi-shot scences.


\begin{figure*}
\centering
\includegraphics[width=0.9\linewidth]{pic/F5.pdf}
\caption{\textbf{QA Generation Pipeline and MultiClip-Bench Examples.}  Questions fall into four types: consistency, short-frame, unexpected content, and others. The video shows children flying kites and running. Type 1 involves person re-identification and discontinuous actions. Type 2 focuses on events between seconds 23-24 (short-frame). Type 3 addresses non-critical background details.}
	\label{fig:3}
\end{figure*}


\begin{figure*}[!t]
	\centering
	\includegraphics[width=0.77\linewidth]{pic/pipeline_last_2.pdf}
\caption{\textbf{The pipeline of Our IPFormer-VideoLLM.}
First, video slices are sampled using a sliding window, and a video encoder extracts visual features from each slice. These features are passed to a visual alignment module, where frame-level and instance-level information are extracted separately. Frame-level information includes cls tokens (classification markers for each frame) and avg pooling tokens (via global average pooling), while instance-level information is generated by an IP Token Generator. Next, frame-level and instance-level information are concatenated and injected into a learnable query through addition to optimize it. The optimized query is fed into an attention mechanism for feature fusion, and the fused features are projected through an MLP for text alignment. Finally, the aligned visual features from all video segments are combined with text features and input into a large language model (LLM) for further processing.}

	\label{fig:pipeline}
\end{figure*}
\vspace{-5pt}
\noindent\subsection{QA Pairs of Multi-Shot Scenes}
\label{3.2}
% During multi-shot transitions, we face challenges that can be broadly categorized into three types:
% \textbf{1.consistency understanding:} Cross-shot character consistency requires re-identification of characters in discontinuous visual contexts, covering: Temporal Action Association: Tracking action continuity after interruptions, such as action counting, temporal Action Understanding. Dynamic Identity Counting: Accurately counting the number of characters before and after shot transitions.
% \textbf{2. short frame understanding:}Instantaneous scene perception, addressing modeling deficiencies for short visual cues (less than 3 seconds): The model's attention mechanism tends to overlook semantically critical frames during rapid shot changes.
% \textbf{3.unexpected
% content} Challenges that deviate from mainstream understanding, which can be regarded as xpected content appearing in multi-shot scenarios that does not align with mainstream content. Such content is also  easily overlooked due to its deviation from conventional patterns.

%\wzc{
After obtaining the key elements for describing multi-shot videos, the next step is to generate suitable QA pairs for training and testing sets. In addition to enhancing instruction-following capabilities, QA pairs can also improve comprehension abilities. The generation process and examples are shown in the Figure~\ref{fig:3}.

We first explore the challenges of understanding multi-shot videos, which can be generally categorized into three types. QA pairs are generated for each of these challenge types: \textbf{i) Consistency Understanding.} The main focus is on identifying the same characters in non-consecutive keyframes. In particular, this QA type includes but is not limited to, tracking action continuity, such as action counting, temporal action understanding, and character number counting. \textbf{ii) Short Frame Understanding.} This challenge involves addressing modeling deficiencies in capturing the visual cues of keyframes in brief moments. To solve the challenge, questions are posed around these frames, focusing on visual issues such as instantaneous actions, appearance information, and other visually relevant details. \textbf{iii) Unexpected Content Understanding.} The core focus is on handling content that deviates from the main theme, i.e., non-critical unexpected content in multi-shot scenes that does not align with the main video context, which we refer to as ``unexpected content." The questions focus on the individuals and objects appearing in these non-critical, unexpected scenes. These three categories comprehensively address the main challenges of multi-shot transitions.

With the proposed QA types, we employ GPT-4 to create 10 QA pairs per video, focusing on multi-person scenes with shot transitions. Then we pass the generated initial QA pairs to GPT-4 for refinement, where 4 to 6 high-quality QA pairs are retained. Finally, three incorrect options are added to each question, converting them into a multiple-choice format with GPT-4. The videos are sourced from the collection in the previous stage. The training set contains $45.5$k video-text pairs, and the test set contains $2.75$k video-text pairs, with no overlap between the two sets. The manually curated, corrected, and categorized test set includes $800$ consistency understanding questions, $703$ unexpected content understanding questions, $562$ short-frame understanding questions, and $685$ other questions covering fine-grained tasks and general comprehension.








 




==> ICCV2025-Author-Kit-Feb/sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> ICCV2025-Author-Kit-Feb/sec/4_Method_4.tex <==
\label{sec:intro}

\section{Visual-Prompt Former for Video LLM}
In addition to the MultiClip-Bench, we propose IPFormer-VideoLLM, which is adapted for multi-shot video understanding. 
This section details the design and structure of IPFormer-VideoLLM. Section \ref{Pipeline of IPFormer-VideoLLM} describes the model architecture. Section \ref{Vision Compressor of IPFormer} discusses the Vision Alignment module. Section \ref{IP Token Generator} introduces the setup of our Visual-prompt tokens.




\subsection{Pipeline of IPFormer-VideoLLM} \label{Pipeline of IPFormer-VideoLLM}
%\wzc{
IPFormer-VideoLLM, built on Video-LLaVA, consists of three main modules as illustrated in Figure~\ref{fig:pipeline}: a visual encoder, a visual alignment module (incorporation the IP Token Generator, attention mechanism and MLP), and a large language model (LLM). Due to the fixed number of frame constraint for video encoders, we employ a sliding-window sampling approach. %This method improves the capture of local information compared to encoding entire video at once. 
Specifically, for an input video, $F$ frames are uniformly extracted. Using a sliding window of $8$ frames, we perform non-overlapping sampling, resulting in $T = \left\lfloor \frac{F}{8} \right\rfloor$ slices. Each slice is processed separately by the visual encoder and the visual alignment module. The processed slices are then concatenated and fed into the LLM along with the text. One significant improvement over previous methods is the visual alignment module, where instance feature tokens generated by the IP Token Generator are used as prompts to guide the attention mechanism in aggregating instance features.


% Our model, illustrated in Figure~\ref{fig:pipeline}, consists of three main modules: a visual encoder, visual alignment (with IP Token Generator, attention and MLP), and a large language model (LLM). It is built on Video-LLaVA~\cite{lin2023video} as the baseline. The visual processing block (visual encoder and visual alignment) uses a sliding-window sampling approach, compatible with video encoders that process a fixed number of frames. This method improves the capture of localized information compared to encoding entire video segments at once. For an input video, $F$ frames are uniformly extracted. Using a sliding window of $8$ frames, we perform nonoverlapping sampling across these frames, resulting in $T = \left\lfloor \frac{F}{8} \right\rfloor$ slices. Each slice is processed separately by the visual encoder and visual alignment. The processed slices are then concatenated and fed into the LLM along with the text. Among our improvements over previous methods is the visual alignment module, where the instance feature tokens generated by the IP Token Generator are used as prompts to guide the attention mechanism in aggregating instance features.




% Our model is shown in Figure~\ref{fig:pipeline}.  Similar to typical models, our model consists of three main modules: a visual encoder, visual alignment (with IP Token Generator), and a large language model (LLM).   Our model is based on Video-LLaVA~\cite{lin2023video} as the baseline.Visual processing block (visual encoder, visual alignment) adopts a sliding-window sampling approach, which is compatible with video encoders that process a fixed number of frames (typically 8 frames). Moreover, compared to encoding the entire video segment at once, learning in smaller chunks allows for better capture of localized information within each segment.  Specifically, for the input video, we evenly divide it into $S$ frames. Our visual sliding window is sized for 8 frames, and we perform non-overlapping complete coverage sampling on these $S$  frames, which means we sample $T = \left\lfloor \frac{F}{8} \right\rfloor$ times, resulting in $T$  slices. For each slice, we process it separately using the visual encoder and visual compressor.  After processing, the $T$  slices are concatenated and fed into the LLM along with the text. 

\subsection{Vision Alignment Module of IPFormer} \label{Vision Compressor of IPFormer}

% \wzc{\textbf{Motivation} Based on our research on data, we assume that a projector for multi-shot video understanding should meet two requirements: (1) Effectively compression ability for vision token, it should be able to handle lots of frames. (2) Instance aware ability, which means it can capture important instance information across scenes. However, current video projector often overlook the importance of instance.
% Inspired by these two requirements, we propose an instance-based compressor. Besides, incorporating instance information helps in capturing more effective video information, thereby achieving more efficient compression capabilities empirically.}

\textbf{Motivation: }Based on our research on data, we assume that visual alignment modules for multi-shot video understanding should meet two requirements: i) Effective compression capability for vision token, allowing them to handle many frames. ii) Instance awareness, enabling the capture of important instance information across scenes. However, current visual alignment modules, whether full projection or compression before projection, encode instance features in a discrete or lossy manner, inevitably losing instance-level information. Inspired by these requirements, we propose an instance-based compressor as a visual alignment module, which reduces key feature loss while compressing visual tokens.%Inspired by these needs, we propose an instance-based compressor that reduces key feature loss while compressing visual tokens.

% Current visual alignment modules, whether projecting full tokens or compressing them before projection, inevitably lose information when aligning video data with text. They also fail to aggregate instance features across multi-shot scenes, relying entirely on LLMs for this task. Although LLMs are powerful, the lossy and fragmented visual features significantly degrade performance in multi-shot scenarios. Our goal is to design a more effective visual compressor that retains key features before inputting data into the LLM, enabling better aggregation of instance features across multi-shot scenes.




  
% We use an external detector to extract all potential instances (including humans and objects) and obtain their instance features. These features are aggregated based on similarity, resulting in instance tokens with meaningful associations. Inspired by Conditional-DETR~\cite{meng2021conditional}, we introduce "anchors"~\cite{ren2015faster,meng2021conditional} during the initialization of learnable queries. The instance feature tokens serve as prompts to guide the attention mechanism in aggregating instance features across different video frames, enhancing contextual associations. Additionally, we incorporate frame-level information to compensate for the lack of global context, particularly in the video encoder and visual compressor. 
\noindent\textbf{Method: }To enable the attention mechanism to capture more critical information, 
we introduce ``anchors"~\cite{ren2015faster,meng2021conditional} during the initialization of learnable query tokens inspired by Conditional-DETR~\cite{meng2021conditional}.
% we are inspired by Conditional-DETR~\cite{meng2021conditional} and introduce ``anchors"~\cite{ren2015faster,meng2021conditional} during the initialization of learnable query tokens. 
These anchors help the learnable tokens extract relevant information from frames, 
% a large amount of data, 
thereby better preserving key information. Thus, we input both instance-level and frame-level information as ``anchors" into the learnable query tokens. 
% Our critical information consists of instance-level information, and in addition, we also incorporate frame-level information to supplement the frame context. Thus, we input both instance-level and frame-level information as``anchors" into the learnable query tokens.
Specifically, 
% for video encoder and visual compressor. 
prior to encoding, the video is pre-processed into images of size $224 \times 224$ for 8 frames. The video encoder then processes these 8 frames into $\mathbf{R} \in \mathbb{R}^{8 \times N \times D}$, where $N$ is the number of tokens per frame, and $D$ is the vector dimension. Here, $N = 256 + 1$, where $256$ denotes the number of image tokens per frame, called $\mathbf{N}_I \in \mathbb{R}^{256 \times D}$, and $1$ is the class token per frame, referred to as $\mathbf{C} \in \mathbb{R}^{1 \times D}$. Next, global average pooling in performed on $\mathbf{N}_I$ to obtain the global feature of each frame, $\mathbf{GF} \in \mathbb{R}^{1 \times D}$.  We use $\mathbf{GF}$ and $\mathbf{C}$ as global information for each frame (frame-level guidance). To enhance frame information learning,  $\mathbf{GF}$ and $\mathbf{C}$ are repeated each $X$ times ($X$=$5$), then concatenated to obtain the frame token for each frame: $\mathbf{FT} = (\mathbf{C} \times X, \mathbf{GF} \times X) \in \mathbb{R}^{(X \times 2) \times D}$. 
In addition, we also obtain instance features through the IP Token Generator. The instance prompt tokens for this segment are represented as $\mathbf{IP} \in \mathbb{R}^{V \times D}$, where $V$ is the number of instance tokens. We concatenate $\mathbf{FT}$ of $8$ frames and $\mathbf{IP}$, resulting in the visual tokens for 8 frames as $\mathbf{VT} \in \mathbb{R}^{8 \times (X \times 2 ) \times D+ V\times D}$. Finally, $\mathbf{VT}$ is added to the learnable queries to optimize them, guiding the learnable queries to aggregate the video features in the cross-attention mechanism, thereby better capturing relevant instance or other useful information. The output of the attention is then projected using an MLP to align with the textual space.
%Finally, the object query is formulated as $\mathrm{add}(\mathbf{VT}, \text{learnable token})$ and sent into cross-attention for feature blending, then projected using MLP.


%Besides, each frame is then processed by an external detector~\cite{zhu2020deformable,ma2024groma} to detect potential instances, with ROI features of these instances aggregated to get the instance feature, and we then perform similarity  clustering on the instance features of a slice (8 frames) to obtain instance prompt token (IP token). This step is mainly beneficial for aggregating multiple similar instances (e.g., similar poses of the same person may appear multiple times in this slice). Finally, the instance prompt token, for this slice are obtained as $\mathbf{IP}$,expressed as $\mathbf{IP} \in \mathbb{R}^{V \times D}$, where $V$ is the number of instance tokens per slice.



\subsection{IP Token Generator} \label{IP Token Generator}
The IP Token Generator generates instance tokens as prompts. Specifically, we employ a category-agnostic detector \cite{zhu2020deformable}, with initialization parameters derived from~\cite{ma2024groma}. The detector's original classification head is replaced by a binary classifier to score region proposals based on their localization quality. This process yields a series of bounding boxes, which are subsequently processed through Non-Maximum Suppression~\cite{neubeck2006efficient}. 
For each frame, we retain only $M$ (fewer than $10$) candidate boxes, truncating any excess and padding with zeros when necessary. 
These candidate boxes are processed using global RoI pooling on the visual feature maps of each frame to obtain instance features. Subsequently, we compute the cosine similarity between the instance features across all frames within a video slice. We set a threshold ($0.9$) %and adopt a strategy akin to depth-first search for aggregation. Starting from the first ungrouped instance, we recursively gather all instances with similarities exceeding the threshold to form a group. Subsequent rounds of traversal are conducted until no further groupings can be formed. Any residual instances failing to meet the similarity criteria ultimately form independent groups. 
 and adopt an iterative grouping strategy. Starting from the first ungrouped instance, we traverse all remaining ungrouped instances,  gathering those with similarities exceeding the threshold to form a group. Subsequent rounds of traversal are performed until no further groupings can be formed. Any residual instances failing to meet the similarity criteria ultimately constitute independent groups. For each group, the channel-wise average is computed to obtain aggregated instance features, referred to as the Instance Prompt. The number of Instance tokens per slice is limited to a maximum of $V$ ($80$), with zeros padded when fewer than $80$ tokens are present. The purpose of clustering is to balance the number of instances, preventing instances that appear frequently from overwhelming sparse ones. This approach is particularly beneficial for short frame understanding.






==> ICCV2025-Author-Kit-Feb/sec/5_Exp.tex <==
\section{Experiments}



\begin{table}[htbp]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt} % 更小的间距
\renewcommand{\arraystretch}{1.0}
\resizebox{\linewidth}{!}{ % 让表格自适应页面宽度
\begin{tabular}{@{}lccccc@{}}
\hline
Method      & Frame & Token & Train Time & FPS & Act-Net \\
\hline
\rowcolor{blue!5}Video-LLaVA & 8 & 2056 & 41h & 1.1 & 45.3 \\
\hline
Ours (8f) & 8 & 160 & 10h & 3.3 & 45.5 \\
Ours (16f) & 16 & 320 & - & 2.0 & 46.1 \\
\hline
\end{tabular}
}
\caption{Efficiency comparison between Video-LLaVA and ours. The highlighted row in \textcolor{blue!30}{blue} is our baseline model.}\label{tab:1}
\end{table}



 \begin{table*}\small
 \centering
 \renewcommand{\arraystretch}{1}
\addtolength{\tabcolsep}{1pt}
 {
\begin{tabular}{@{}l|c|c|c|cccc|c@{}}
\hline
% Image     & b& P  & \multicolumn{7}{c}{SNR}  \\
% \cline{4-11}
Method & LLM size &Frames& Tokens &Consistency uds &Short uds&Unexpected content&Others  &Mean \\ \hline
\rowcolor{blue!5} Video-LLaVA~\cite{lin2023video} &7B & 8 &2056 &32.9&40.0 & 46.2&60.7& 44.5 \\
VideoChat2~\cite{li2024mvbench}  &7B & 16&96& 33.4& 32.3 &47.6  & 58.1& 42.9\\
ST-LLaVA~\cite{qu2024ts}  &7B  & 100 &2304&31.1&38.8&48.3  &56.8&43.5 \\

PLLaVA~\cite{xu2024pllava} &7B  & 16 &2304&36.5&43.0 &55.9 &63.2&49.4\\ 
LLaVA-MINI~\cite{zhang2025llava}&8B   & 64 &64&26.8& 40.9& 53.2&58.6&44.9\\ 



 \hline
 \textbf{Ours} (w/o MultiClip) & 7B &  16&320 &37.7&43.1& 48.4&61.9&48.1\\ 
 \textbf{Ours} & 7B&  16&320&46.1 &53.6&60.4&66.3&57.0\\ 
  \textcolor{DarkGreen}{\textbf{$\Delta Acc$}.}
 & -&  -&- &\textcolor{DarkGreen}{\textbf{+8.4}}&\textcolor{DarkGreen}{\textbf{+10.5}}& \textcolor{DarkGreen}{\textbf{+12.0}}&  \textcolor{DarkGreen}{\textbf{+4.4}}& \textcolor{DarkGreen}{\textbf{+8.9}}  \\ 
 \textbf{Ours} &7B &  48&960&\textbf{48.6}& \textbf{56.7}& \textbf{62.5}&68.5&\textbf{58.8}\\ 
  \hline
  GPT-4o-mini~\cite{abacha2024medec}   &8B &16&Unk & 44.7&44.6 &55.3 &59.1 & 50.9\\
GPT-4V\cite{yang2023dawn}   &Unk &8&Unk &34.6&31.5 &45.3  &52.4 & 41.8 \\
  Qwen2.5-vl~\cite{bai2025qwen2}    &72B&16&Unk &43.5&\textbf{58.3} & \textbf{62.4} &72.8 &58.5\\ 
Gemini-1.5-pro~\cite{team2024gemini}  &Unk & 16&Unk&\textbf{53.4} & 52.5& 62.0 &\textbf{74.4} & \textbf{60.5}\\

\hline
\end{tabular}
}
\caption{Comparison with other models on MultiClip-Bench. Best performance is \textbf{boldface}. The highlight in \textcolor{blue!30}{blue} is our baseline model.}
\label{tab:2}%
\end{table*}




\begin{table}[t]
    \centering
    \footnotesize
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}lc|ccc@{}}
        \hline
        \multirow{2}{*}{Method}  & \multirow{2}{*}{LLM Size} 
        & \multicolumn{3}{c}{\textbf{QA Metrics}} \\
        \cline{3-5}
        & & MSVD & MSRVTT & ActivityNet \\ 
        \hline
        FrozenBiLM~\cite{yang2022zero}  & 1.3B & 33.8 & 16.7 & 25.9 \\
        Video-LLaMA~\cite{zhang2023video} & 7B & 51.6 & 29.6 & 12.4 \\
        LLama-Adapter~\cite{zhang2023llama}  & 7B & 54.9 & 43.8 & 34.2 \\
        Video-ChatGPT~\cite{maaz2023video}& 7B & 64.9 & 49.3 & 35.3 \\
        VideoChat~\cite{li2023videochat} & 7B & 56.3 & 45.0 & 26.5 \\
        \rowcolor{blue!5}  Video-LLaVA~\cite{lin2023video}&7B & 70.7 & 59.2 & 45.3 \\
        Chat-UniVL~\cite{jin2024chat}  &7B & 65.5 & 54.6 & 45.8 \\
        MovieChat~\cite{song2024moviechat} & 7B & 75.2 & 52.7 & 45.7 \\
        VideoChat2~\cite{liu2024mmbench} &7B & 70.0 & 54.1 & 49.1 \\
        Vista-LLama~\cite{ma2023vista} & 7B & 65.3 & 60.5 & 48.3 \\
        LLAMA-VID\cite{li2024llama} & 13B & 70.0 & 58.9 & 47.5 \\
        ST-LLM~\cite{liu2024st}& 7B & \textbf{74.6} & \textbf{63.2} & \textbf{50.9} \\
        \hline
        Ours & 7B & 73.8 & \textbf{63.2} & 50.1 \\
        \hline
    \end{tabular}
    }
    \caption{Quantitative comparison on video question-answering.}
    \label{tab:results_video_qa}
\end{table}

\begin{table}[h]
\footnotesize
\addtolength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}
{
\begin{tabular}{@{}l|c|c|c@{}}

\hline
\textbf{Method} & \textbf{Vision Encoder} & \textbf{LLM Size} & \textbf{Avg.} \\ \hline
Video-LLaMA \cite{zhang2023video} & CLIP-G & 7B & 34.7 \\
LLaMA-Adapter \cite{zhang2023llama} & ViT-B & 7B & 31.7 \\
Video-ChatGPT \cite{maaz2023video} & ViT-L & 7B &  32.7 \\
VideoChat\cite{li2023videochat}  & CLIP-G & 7B &35.5 \\
\rowcolor{blue!5}  Video-LLaVA\cite{lin2023video}  &ViT-L&7B& 42.2 \\
VideoChat2 \cite{li2024mvbench} & UMT-L & 7B & \textbf{51.1} \\
PLLaVA  \cite{xu2024pllava} & ViT-L & 7B & 46.5 \\
LLaVA-MINI \cite{zhang2025llava}  & ViT-L&8B & 44.5 \\

\hline
Ours     &ViT-L&7B & 48.3 \\ 
\hline
\end{tabular}
}
\caption{Quantitative comparison on MVBench.}
\label{tab:mvbech}
\end{table}



% \begin{table}[h]
% \footnotesize
% {
% \begin{tabular}{l|c|c|c}
% \hline
% \textbf{Method} & \textbf{Vision Encoder} & \textbf{LLM Size} & \textbf{Avg.} \\ \hline
% Video-LLaMA \cite{50} & CLIP-G & 7B & 30.7 \\
% LLaMA-Adapter \cite{51} & ViT-B & 7B & 31.7 \\
% Video-ChatGPT \cite{33} & ViT-L & 7B &  32.7 \\
% VideoChat  &  & 7B &35.5 \\

% VideoChat2 \cite{20} & UMT-L & 7B & 51.1 \\
% PLLaVA  & ViT-L & 7B & 46.5 \\
% LLaVA-MINI  & ViT-L & 44.5 \\
% Video-LLaVA\cite{19}  & 35.5 \\
% \hline
% Ours     &ViT-L&7B & 48.3 \\ 
% \hline
% \end{tabular}
% }
% \caption{Results on MVBench multi-choice question answering.}
% \label{tab:mvbech}
% \end{table}


\begin{table}\footnotesize
    \centering
    \addtolength{\tabcolsep}{8pt}
    
    \begin{tabular}{@{}l|c|c|c@{}}
        \hline
        Method  & NExT-QA & Egoschema &IntentQA \\
        \hline
        \rowcolor{blue!5} Video-LLaVA \cite{lin2023video}   & 60.5 & 37.0& -\\
        Video-LLaMA2 \cite{cheng2024videollama}   & - & 51.7 &- \\
        MovieChat+ \cite{song2024moviechat}   & 54.8 & 56.4 &- \\
        Vista-LLaMA \cite{ma2023vista}   & 60.7 & - & - \\
        DeepStack-L \cite{meng2025deepstack}   & 61.0 & 38.4  &-\\
        M$^3$ \cite{cai2024matryoshka}  & 63.1 & 36.8  &58.8\\
        IG-VLM \cite{kim2024image}   & 63.1 & 35.5  &60.3\\
        SF-LLaVA \cite{xu2024slowfast}  & 62.4 & 47.6 & 60.1\\
        TS-LLaVA \cite{qu2024ts}  & 66.5 & \textbf{50.2}& 61.7\\
        \hline
        ours   &  \textbf{70.6}& 50.0 & \textbf{75.3}\\
        \hline
    \end{tabular}
    \caption{Quantitative comparison on Multiple-choice question-answering in specific fields.}
    \label{tab:multiple_choice}
    \label{tab:results}
\end{table}
% \begin{table}[!t]\small
% \centering
% \renewcommand\arraystretch{1}
% % \addtolength{\tabcolsep}{1pt}
% \resizebox{85mm}{15mm}
% {
% \begin{tabular}{@{}lcccccc@{}}
% \hline
% % Image     & b& P  & \multicolumn{7}{c}{SNR}  \\
% % \cline{4-11}
% method& backbone &shot1-Mean &shot2-Mean
% \\ \hline
% SCAPE+& ViT-b & $88.19$  & $91.53$\\
% SCAPE+&  Swin-b &\\
% SCAPE+&  ViT-s(DINOv2) &$90.74$& $92.65$\\
% SCAPE+&  ViT-b(DINOv2)  & $91.95$ & $93.98$ \\
% CapeFormer &ViT-b(DINOv2) & $89.11$ &  $91.91$ \\

% \hline
% \end{tabular}
% }
% \caption{Performance Across Different Transformer-Based Backbones, we report averages across 5 splits on the MP-100 dataset, considering both 1-shot and 5-shot settings.}\label{tab:dif}
% \end{table}


% \begin{table}[!t]\small
% \centering
% \renewcommand\arraystretch{1.3}
% % \addtolength{\tabcolsep}{1pt}

% \centering
% \renewcommand\arraystretch{1}
% \resizebox{80mm}{7mm}
% {
% \begin{tabular}{@{}lcccccc@{}}
% \hline
% % Image     & b& P  & \multicolumn{7}{c}{SNR}  \\
% % \cline{4-11}
% Method& split1 &split2    &split3 &split4 &split5 &Mean
% \\ \hline
% CapeFormer &$0.088/88.64$ & & &  \\
% SCAPE+& \\
% \hline
% \end{tabular}
% }
% \caption{Comparison with state-of-the-art approach es on the MP-100 dateset in terms of NME and AUC}\label{tab:NME}
% \end{table}





%------------------------------------------------------


% \begin{table*}[h]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|c|c|ccccccccccccccccccccc}
% \hline
% \textbf{Method} & \textbf{Vision Encoder} & \textbf{LLM Size} & \textbf{AS} & \textbf{AP} & \textbf{AA} & \textbf{FA} & \textbf{UA} & \textbf{OE} & \textbf{OI} & \textbf{OS} & \textbf{MD} & \textbf{AL} & \textbf{ST} & \textbf{AC} & \textbf{MC} & \textbf{MA} & \textbf{SC}& \textbf{FP}& \textbf{CO}& \textbf{EN}& \textbf{ER} & \textbf{CI}& \textbf{Avg.} \\ \hline
% Video-LLaMA \cite{50} & CLIP-G & 7B & 27.5 & 28.5 & 51.0 & 29.0 & 39.0 & 48.0 & 45.0 & 38.0 & 22.5 & 22.5 & 43.0 & 34.0 & 22.5 & 32.5 & 45.5 & 30.7 \\
% LLaMA-Adapter \cite{51} & ViT-B & 7B & 23.0 & 28.0 & 61.0 & 30.0 & 30.5 & 53.5 & 32.5 & 32.5 & 21.0 & 25.0 & 21.5 & 30.5 & 29.0 & 23.5 & 41.5 & 31.7 \\
% Video-ChatGPT \cite{33} & ViT-L & 7B & 23.0 & 26.0 & 62.0 & 29.0 & 34.0 & 55.0 & 54.0 & 28.0 & 40.0 & 20.0 & 30.5 & 29.5 & 28.5 & 30.0 & 45.5 & 32.7 \\
% VideoChat  &  & 7B & 33.5 & 26.5 & 65.0 & 20.0 & 47.5 & 70.5 & 52.0 & 40.5 & 30.0 & 25.5 & 27.0 & 48.5 & 30.5 & 42.0 & 46.0 & 35.5 \\

% VideoChat2 \cite{20} & UMT-L & 7B & 31.5 & 28.0 & 83.5 & 49.5 & 36.0 & 58.0 & 71.5 & 42.0 & 44.5 & 27.0 & 23.5 & 40.5 & 36.0 & 49.0 & 43.5 & 51.1 \\
% PLLaVA  & ViT-L & 7B & 58.0 & 49.0 & 55.5 & 41.0 & 61.0 & 61.0 & 36.0 & 33.5 & 25.5 & 26.0 & 28.0 & 43.0 & 28.5 & 42.0 & 52.0 & 46.5 \\
% LLaVA-MINI  & ViT-L & 7B & 58.0 & 49.0 & 55.5 & 41.0 & 61.0 & 61.0 & 36.0 & 33.5 & 25.5 & 26.0 & 28.0 & 43.0 & 28.5 & 42.0 & 52.0 & 44.5 \\
% Video-LLaVA\cite{19} & CLIP-G & 7B & 33.5 & 26.5 & 65.0 & 20.0 & 47.5 & 70.5 & 52.0 & 40.5 & 30.0 & 25.5 & 27.0 & 48.5 & 30.5 & 42.0 & 46.0 & 35.5 \\
% \hline
% Ours     &ViT-L&7B & 59.5 & 51.5&84.5&41.5&59.5 &57.5&56.0&31.5&23.0&27.0&80.5 & 46.5 & 48.5 &49.5 & 57.5 & 26.0 & 38.0 &33 & 48 &47.5& 48.3 \\ 
% \hline
% \end{tabular}
% }
% \caption{Results on MVBench multi-choice question answering.}
% \label{tab:mvbech}
% \end{table*}

\subsection{Implementation Details} 


\noindent \textbf{Model Details: }To validate the effectiveness of the proposed modules, we use Video-LLaVA~\cite{lin2023video} as the baseline, maintaining the same training settings to ensure the only difference are in the model modifications. Specifically, visual encoder from LanguageBind~\cite{zhu2023languagebind} is used, initialized from OpenCLIP-L/14~\cite{radford2021learning}, with a resolution of 224×224. For large language model, we use the LLM in LanguageBind initialized from Vicuna-7B v1.5~\cite{zheng2023judging}. The text tokenizer is from LLaMA~\cite{touvron2023llama} with about 32,000 classes. 

Regarding our design, in addition to the two-layer MLP full projection with GeLU~\cite{hendrycks2016gaussian} for the visual compressor, we adopt the approach of BLIP2~\cite{li2023blip} and VideoChat2~\cite{li2024mvbench}, implementing an attention parameter compression module using pre-trained BERTbase~\cite{devlin2019bert}. For the external detector, we adopt the Region Proposer parameters from Groma~\cite{ma2024groma}, implementing a modified binary classifier based on Deformable DETR~\cite{zhu2020deformable}.


% To validate the performance improvements at the model level, we use Video-LLaVA~\cite{lin2023video} as the baseline while keeping the same experimental configurations. Specifically, we use visual encoders from LanguageBind~\cite{zhu2023languagebind}, which is initialized from OpenCLIP-L/14~\cite{radford2021learning} with 224×224 resolutions. 
% %Visual encoders we default to use visual encoders are derived from LanguageBind~\cite{zhu2023languagebind}, initialized from OpenCLIP-L/14~\cite{radford2021learning} with 224×224 resolutions. 
% For large language model, we still the LLM in LanguageBind initialized from Vicuna-7B v1.5~\cite{zheng2023judging}. LLaMA~\cite{touvron2023llama} is employed as the text tokenizer, with approximately 32,000 classes.  
% %The text tokenizer is from LLaMA~\cite{touvron2023llama}, with approximately 32,000 classes.  
% In addition to the two-layer MLP full projection with GeLU~\cite{hendrycks2016gaussian} for the visual compressor, we follow the approach of BLIP2~\cite{li2023blip} and VideoChat2~\cite{li2024mvbench} by implementing an attention parameter compression module using pre-trained BERTbase~\cite{devlin2019bert}. For the external detector, we adopt the Region Proposer parameters from Groma~\cite{ma2024groma}, implementing a modified binary classifier based on Deformable DETR~\cite{zhu2020deformable}.

% \noindent \textbf{Visual Encoder and Large Model} To validate the adaptation of our approach to setting, We conduct experiments using our method under the different settings of Video-LLava[]. For visual encoder and LLM, we following Video-LLava[], we apply the  OpenCLIP-L/14[]  with 224×224 resolutions and Vicuna-7B v1.5[]: . 


% \noindent \textbf{External detector} We follow Groma[], utilize the Deformable DETR (DDETR)[] transformer [] to extract feature maps from the last four layers of the image encoder. These feature maps are then rescaled to construct a hierarchical feature pyramid for input to the region proposer. For each image, the region proposer generates $300$ region proposals. We set the NMS threshold to $0.6$ and filter out region proposals with an objectness score below $0.15$.
% \vspace{5pt}


\noindent\textbf{Training Details: }Our training process follows Video-LLaVA~\cite{lin2023video} and is divided into two stages: modality alignment pretraining and instruction fine-tuning. 
% To validate our propositions, we adopt the same training settings as the baseline (including the pre-trained model, data, and parameters). %he specifics are as follows:

% During the pretraining stage, we use the same training data as  Video-LLaVA, including $558$K image-text pairs from LAION-CC-SBU~\cite{liu2023visual,sharma2018conceptual} and $702$K video-text pairs from Valley~\cite{luo2023valley}. The training process involves random combinations of images and videos in each batch. For each video, we uniformly sample $8$ frames, with each frame resized and cropped to $224 \times 224$. The training focuses on the visual alignment module, while keeping other parameters frozen and only training the visual compression module (both attention and full projection modules). We employ the AdamW optimizer with cosine learning rate scheduling, setting the learning rate to $1e-3$ and a warmup ratio of $0.03$. The training runs for one epoch with a batch size of $256$.
During \textit{modality alignment pretraining}, we follow Video-LLaVA using $558$K image-text pairs from LAION-CC-SBU~\cite{liu2023visual,sharma2018conceptual} and $702$K video-text pairs from Valley~\cite{luo2023valley}. We train the visual alignment module for one epoch (batch size 256) using AdamW optimizer (lr=$1e^{-3}$, warmup=$0.03$), while freezing other parameters. Each video contains $8$ frames at a $224 \times 224$ resolution.


% In the second stage, we also adhere to all experimental settings of Video-LLaVA. Specifically, we use the 665K image-text instruction dataset from LLaVA-v1.5~\cite{liu2024improved} and the 100K video-text instruction dataset from Video-ChatGPT~\cite{maaz2023video}, sampling 8 frames from each video (consistent with Video-LLaVA) to evaluate model improvements. In the experiments, only the video encoders are frozen, while the LLM is fine-tuned with all parameters. The batch size was set to $128$, while all other settings remained consistent with the previous stage. After training, the relative improvements of the model can be found in Tables~\ref{tab:1}~\ref{tab:5}~\ref{table:8}.
% In the second stage, we also follow Video-LLaVA's experimental settings, utilizing a dataset containing $665$K image-text instruction pairs from LLaVA-v1.5~\cite{liu2024improved} and $100$K video-text instruction pairs from Video-ChatGPT~\cite{maaz2023video}. Following Video-LLaVA's protocol, we sample $8$ frames from each video for model evaluation. During this phase, while the video encoders remain frozen, we fine-tune all parameters of the LLM. The batch size is set to $128$, with all other hyperparameters maintained from the previous stage. The relative performance improvements of our model are detailed in Tables~\ref{tab:1},~\ref{tab:5}, and~\ref{table:8}.

% To further enhance performance, we first selected $326$K instruction video-text data from VideoChat2~\cite{li2024mvbench}, and added $27$K data from the Perception\cite{patraucean2023perception} and STAR~\cite{wu2024star} training sets. To adapt to multi-shot scences, we introduced the proposed MultiClip training set, which contains $68$K video-text data, and increased the number of training frames to $16$ (sampled twice using a sliding window approach). 
For the \textit{instruction tuning} stage, we use the same base data as Video-LLaVA ($665$K image-text pairs from LLaVA-v1.5 and $100$K video-text pairs from Video-ChatGPT). To further enhance performance, we additionally selected $326$K instruction pairs from VideoChat2~\cite{li2024mvbench}, $27$K data from Perception~\cite{patraucean2023perception} and STAR~\cite{wu2024star} datasets, and $68$K video-text pairs from our MultiClip dataset. We also increase the number of sampled frames from 8 to 16 using a sliding window approach to benefit multi-shot scenes. The training settings remain consistent with Video-LLaVA: keeping video encoders frozen while fine-tuning all LLM parameters with a batch size of 128.



% In the second stage, to test the pure improvement of our model, we maintain the same settings as the baseline. We use the 665K image-text instruction dataset from LLaVA v1.5 [] and the 100K video-text instruction dataset from Video-ChatGPT []. We only freeze the image/video encoders. To ensure fairness, we sample 8 frames from videos (consistent with Video-LLaVA) to evaluate the model's improvement. We reduce the batch size to $128$, while all other experimental parameter settings fully follow Video-LLaVA[].

% To adapt to our multi-shot scenarios, we add more datasets and increase the number of training frames to 16 (using a sliding window approach twice). To further enhance performance, we select 326K instruction video-text data from the 768K training set proposed by VideoChat2 and 27K of the data comes from Perception[] and Charades[] training set. Then we adopt 68K video-text data from our MultiClip-Bench. This includes three key elements: video description, instruction-based question answering, and more details are provided in the data section as described.



\subsection{Efficiency of IPFormer-VideoLLM}
% The proposed attention-based visual compressor replaces the fully connected layers in Video-LLaVA, significantly reducing visual tokens. Training and inference time costs are detailed in Table ~\ref{tab:1}. The model improves training efficiency while maintaining strong performance. Under identical hardware (8×A100-80G GPUs) and experimental settings, the training time of the first stage is reduced to 1/4, shortening the entire process from 3–4 days to 1–2 days. The test results were obtained on a 3090 Ti. In the figure above, inference and training time of IPformer-VideoLLM exclude box detection (using boxx as label input). With 16-frame inference, including box detection, the speed is 1.4 FPS, still retaining its advantage. 

% To address the computational bottleneck in Video-LLaVA's visual processing, we propose an attention-based visual compressor to replace its fully connected layers. Here we validate its efficiency, reflected in the training and inference time cost in Table ~\ref{tab:1}. The results shows that this modification significantly reduces visual tokens while maintaining model performance. Specifically, under same hardware (8×A100-80G GPUs) and experimental settings, the training time of the first stage is reduced to 1/4, shortening the entire process from 3–4 days to 1–2 days. The test results were obtained on a 3090 Ti. In the figure above, inference and training time of IPformer-VideoLLM exclude box detection (using boxx as label input). With 16-frame inference, including box detection, the speed is 1.4 FPS, still retaining its advantage. 

To address the computational bottleneck in Video-LLaVA's visual processing, we propose replacing its fully connected layers with an attention-based visual compressor. We validate its efficiency through comprehensive timing experiments, as shown in Table~\ref{tab:1}. The results demonstrate that this modification significantly reduces visual tokens while maintaining model performance. Specifically, under the same hardware configuration (8×A100-80G GPUs) and experimental settings, our approach reduces the first-stage training time to 1/4 of the original duration, shortening the entire training process from 3–4 days to 1–2 days. For inference evaluation (conducted on a single 3090Ti), while the timing results in Table~\ref{tab:1} exclude box detection time (as we use pre-computed box labels), our model still achieves 1.4 FPS with 16-frame processing even when including real-time box detection, demonstrating strong computational efficiency. In subsequent experiments, unless otherwise specified, inference is performed with \textbf{$16$} frames by default.





\subsection{Result on MultiClip-Bench}
% We compared our model with existing open-source video multimodal models using our self-constructed Multiclip-Bench dataset, with results shown in Table ~\ref{tab:2}. Experiments demonstrate that our model outperforms the baseline by \textcolor{DarkGreen}{\textbf{+3.6}}; with the support of our proposed training set, the performance significantly improves by \textcolor{DarkGreen}{\textbf{+8.9}}, and increasing the number of video frames further enhances results. Additionally, we evaluated several state-of-the-art multimodal large models (most of which are closed-source) using a multi-image evaluation approach. The results show that Qwen2.5-VL~\cite{bai2025qwen2} and Gemini-1.5-pro\cite{team2024gemini} perform exceptionally well, each excelling in their respective areas of strength.

We compare our model with existing open-source video multimodal models on our self-constructed MultiClip-Bench dataset, with results shown in Table~\ref{tab:2}. By comparing Video-LLaVA and Ours (w/o MultiClip), it is obvious that our model design leads to a significant improvement (\textcolor{DarkGreen}{\textbf{+3.6\%}}) %on multi-shot scenes. %, and more importantly, it only lies in the model change, not about dataset. 
When incorporating our proposed training dataset, performance improves further by \textcolor{DarkGreen}{\textbf{+8.9\%}}. Additionally, increasing the frame number can help understanding. 


We also test several state-of-the-art large multimodal models (most of them are closed-source) using a multi-image evaluation approach. Among these, Qwen2.5-VL~\cite{bai2025qwen2} and Gemini-1.5-pro~\cite{team2024gemini} each demonstrate their strengths in different categories.

% The experiments show that our model improvements alone yield a \textcolor{DarkGreen}{\textbf{+3.6}} performance gain over the baseline. When incorporating our proposed training dataset, the performance further improves by \textcolor{DarkGreen}{\textbf{+8.9}}, with additional gains achieved by increasing the number of video frames. We also benchmark several state-of-the-art multimodal large models (most of them are closed-source) using a multi-image evaluation approach. Among these, Qwen2.5-VL~\cite{bai2025qwen2} and Gemini-1.5-pro~\cite{team2024gemini} demonstrate superior performance, each showing distinct strengths in different aspects.

% \subsection{Dense Recaption}
% Given the enhanced captioning capabilities of VPformer, we further tested its recaptioning task using the 1K-video Inter4K [] caption dataset. An example is shown in Figure 11. Compared to previous pipelines, our model not only captures better caption details but also exhibits improved instance consistency understanding, and provides better perceptual descriptions of video transitions. This demonstrates VPformer's robust video captioning capabilities, indicating its potential contributions to the generation domain.



\subsection{Results on other video benchmarks}

% We evaluate our trained models with the following video-to-text benchmarks. First, the open-ended
% Video Question Answer (VideoQA) includes MSVD-QA[] MSRVTT-QA [], ActivityQA []. Responses in these question-answering benchmarks typically consist of singleword answers. GPT-3.5 [] is used to evaluate the accuracy (Accuracy, with answers true/false). Shown as Table~\ref{tab:results_video_qa}
% Furthermore, we also use the multi-choice Question Answering benchmark, MVBench[], comprising 20 tasks that demand nuanced temporal comprehension of videos in Table ~\ref{tab:mvbech} (specific performance, refer to the supplementary materials.). And we extend the evaluation of our model to other challenging video benchmarks in \ref{tab:multiple_choice},NExT-QA[], Egoscheme[], IntentQA[].

% We tested several common video benchmarks to demonstrate the versatility of the model.  First, in open-ended Video Question Answering tasks, including MSVD-QA~\cite{chen2011collecting}, MSRVTT-QA~\cite{xu2016msr}, and ActivityNet-QA~\cite{yu2019activitynet}, answers are typically short phrases. Following the Video-LLaVA approach, we used GPT-3.5-turbo to evaluate accuracy, with results in Table ~\ref{tab:results_video_qa}. Second, we evaluated on the general multi-choice benchmark MVBench, which comprises 20 tasks requiring detailed temporal understanding of videos, as shown in Table  ~\ref{tab:mvbech} (see supplementary materials for details). Additionally, we tested more challenging benchmarks (also  multi-choice) like NExT-QA~\cite{xiao2021next}, EgoSchema~\cite{mangalam2023egoschema}, and IntentQA~\cite{li2023intentqa}, with results in Table \ref{tab:multiple_choice}. With improvements from both data and model enhancements, our model significantly outperforms the baseline, particularly excelling in NExT-QA and IntentQA. This is attributed to the inclusion of multi-shot scenes and person-centric questions, which our dataset effectively addresses.


Besides the multi-shot scenes, we also evaluate our model on various video benchmarks to demonstrate its versatility. For open-ended Video Question Answering tasks, including MSVD-QA~\cite{chen2011collecting}, MSRVTT-QA~\cite{xu2016msr}, and ActivityNet-QA~\cite{yu2019activitynet}, where answers are typically short phrases, we follow Video-LLaVA to use GPT-3.5-turbo for accuracy evaluation, with results shown in Table~\ref{tab:results_video_qa}. We also assess performance on MVBench, a comprehensive multi-choice benchmark comprising 20 tasks that require detailed temporal understanding of videos, as presented in Table~\ref{tab:mvbech} (see supplementary materials for details). Furthermore, we validate on more challenging multi-choice benchmarks, including NExT-QA~\cite{xiao2021next}, EgoSchema~\cite{grauman2022ego4d}, and IntentQA~\cite{li2023intentqa}, with results shown in Table~\ref{tab:multiple_choice}. Through combined improvements in data and model architecture, our approach significantly outperforms other methods, particularly in NExT-QA and IntentQA. This superior performance can be attributed to the effective coverage of multi-shot scenes and person-centric questions within our dataset.





\subsection{Ablation study}
This section, we analyze the effect of specific model design and dataset, including the comparison of our visual compression module with other visual alignment methods, the specific design of visual compression module, and the impact of the proposed dataset and frame-increasing strategy.


% This section analyzes the gains from model and dataset optimization, including: (1 a comparison of the visual compression module with other compression schemes; (2 the design of the visual compression module; (3 the impact of different training datasets; and (4 the effect of varying frame configurations. Among these, (1 and (2 demonstrate the advantages at the model level, with all settings and baselines keep consistent. %(3 and (4 present the results obtained by incorporating the optimized dataset.

%demonstrates that the limited instruction data proposed in existing datasets such as VideoChat2 (783K) and VideoChatGPT [] (100K) is insufficient to meet the demands for fine-grained and consistent understanding in real-world scenarios. We present a hierarchical dataset along with associated instruction fine-tuning datasets. Ablation experiments were conducted to evaluate the impact of our proposed datasets. The results indicate that key frame descriptions(11k) within our hierarchical dataset provide significant gains. Additionally, instance description datasets(11k) and detailed description datasets(11k) further enhances performance. Ultimately, the generated instruction fine-tuning dataset enables better adaptation for answering relevant questions.
% \begin{table}\scriptsize
% \centering
% \renewcommand\arraystretch{1}

% \begin{tabular}{cc|ccccc}

% \hline
%   \multicolumn{2}{c|}{Visual Alignment Module} & \multicolumn{4}{c}{Metric} \\ \cline{1-2} 
%  structure & Token &  Activity &MSVD  &MSRVTT&MVBench&MultiCilp   \\ \hline
% Full-projection  & 8*256 &45.3 &70.2&60.2 &42.2&44.5\\
% \hline
% Avg-pooing(2*2)  & 8*64 &45.0 &-&- &41.7&-\\
% QFormer  & 160& 40.9 &-&- &40.1&-\\
%  \hline
% IPformer  & 8*20 &45.5 &71.4&61.8 &42.3&46.8\\
%  \hline
% \end{tabular}
% \caption{Thoken to enhance frame features, which im-218
% proves results when con module operates more efficiently across different settings.}\label{tab:5}
% \end{table}
\begin{table}
\footnotesize
\addtolength{\tabcolsep}{0pt}
\centering
\begin{tabular}{@{}l|c|cc|cc@{}}
\toprule
  & \multirow{2}{*}{Frame Query} &  \multicolumn{2}{c|}{Instance Query}&\multirow{2}{*}{ActivityNet}&\multirow{2}{*}{MultiClip}\\
& & no-cluster& cluster &   & 
\\
\midrule
S$1$ & & & &40.9 &42.3\\
S$2$ &\ding{52} & & &42.6  &43.1\\
\midrule
S$3$& \ding{52} & \ding{52}&&43.6 &44.6\\
S$4$& \ding{52} &&\ding{52} &45.5&46.2 \\
\bottomrule
\end{tabular}
\caption{Design of visual compression module.}
\label{table:8}
\end{table}




\begin{table}\footnotesize
\centering
\renewcommand\arraystretch{1.1}
\addtolength{\tabcolsep}{-3pt}
\resizebox{\linewidth}{!}
{
\begin{tabular}{cc|ccccc}

\hline
  \multicolumn{2}{c|}{Visual Alignment Module} & \multicolumn{4}{c}{Metric} \\ \cline{1-2} 
 structure & Token &  Activity   &MSRVTT&MVBench&MultiClip   \\ \hline
Full-projection  & 8*256 &45.3 &60.2 &42.2&44.5\\
\hline
Avg-pooling (2*2)  & 8*64 &45.0 &- &41.7&-\\
QFormer (S1)  & 160& 40.9 &- &40.1&42.3\\
 \hline
IPFormer (S4) & 8*10+80 &45.5 &61.8 &42.3&46.2\\
 \hline
\end{tabular}
}
\caption{Comparison of different visual alignment methods. Avg-pooling and QFormer are common visual compression techniques.}\label{tab:5}
\end{table}

\begin{table}\footnotesize
\centering
\renewcommand\arraystretch{1}
% \addtolength{\tabcolsep}{1pt}
\addtolength{\tabcolsep}{2pt}

\resizebox{\linewidth}{!}
{
\begin{tabular}{@{}ccccc@{}}
\hline
% Image     & b& P  & \multicolumn{7}{c}{SNR}  \\
% \cline{4-11}
 &Data source  &ActivityNet& MVBench  &MuitiClip
\\ \hline
D$1$&  Video-LLaVA&45.8&43.7&47.1\\
D$2$& +VideoChat2(353k)& 48.6&47.5& 48.1\\
D$3$ &+ MultiClip(68k)&50.1  &48.3& 57.0\\
\hline
\end{tabular}
}
\caption{The effect of training dataset.}\label{tab:4}
\end{table}



\noindent\textbf{Design of the Visual Compression Module: }Here we verify the effect of each design aspect within our visual compression module, with results shown in Table~\ref{table:8}. Comparison of S1 and S2 shows that incorporation of frame queries leads to $1.7\%$ performance gain compared to the original learnable queries in Q-Former. Additionally, injecting instance to queries can further improve the performance, but without clustering, the gain is limited. With clustering of instance tokens, performance increases to $46.2$ on MultiClip.

% We validate the gain characteristics of each design within the IPFormer. In Table~\ref{table:8} Our compression module improves upon the cross-attention-based approach. In S1, learnable queries are crossed with video tokens for LLM input. S2 adds global features from each frame to the query. S3 includes a class token to enhance frame features, which improves results when combined with global tokens. S4, S5, and S6 add object tokens for fine-grained frame details. S4 directly adds object tokens to the query without clustering, while S5 and S6 use k-means clustering and similarity clustering methods. S6, with similarity-based clustering, yields the best results.  




\noindent\textbf{Comparison of Different Visual Alignment Methods:} 
% In Table~\ref{tab:5}, we compare our visual compression module with several common visual alignment methods: full projection (commonly used in Video-LLaVA) minimizes information loss; average pooling (adopted by PLLaVA, LLaVA-Next~\cite{li2024llava}, etc.) has a low compression rate and minimal loss; Qformer (used in VideoChat2, etc.) results in significant information loss. Our guided attention-based compressor better preserves useful information, achieving the best performance across all tested datasets, particularly excelling on our MultiClip-Bench.
We compare our visual compression module with other common methods for visual alignment, with results shown in Table~\ref{tab:5}. Full projection, commonly used in Video-LLaVA, does not compress the tokens and thus minimizes information loss. Average pooling, adopted by PLLaVA, LLaVA-Next~\cite{li2024llava}), has a low compression rate, resulting in only marginal performance drops. In contrast, the original Q-Former (S1 in Table~\ref{table:8}) results in significant information loss, which largely impacts the performance. However, with our query design (S4 in Table~\ref{table:8}), the Q-Former architecture can surpass the full-projection while compressing tokens.





\noindent \textbf{Effect of Dataset:}
To validate the effectiveness of our proposed dataset, we conduct experiments to evaluate its impact on model performance. As shown in Table~\ref{tab:4}, the limited instruction data in %VideoChat2 and 
VideoChatGPT~\cite{maaz2023video} used by Video-LLaVA are insufficient to meet the needs for fine-grained and consistent understanding in real scenarios. By incorporating VideoChat2 instruction data and our proposed dataset, we observe substantial performance improvements, which demonstrate that our keyframe annotation strategy significantly enhances model capabilities. Notably, with only 68k training samples, we achieve significant improvements on the MultiClip benchmark.  We also test the performance changes when using different numbers of frames for training and inference, demonstrating the scalability of the model. 
 (Per supplementary materials)


% \begin{table}
% \centering
% \renewcommand\arraystretch{1}
% \addtolength{\tabcolsep}{3pt}


% \footnotesize 
% {
% \begin{tabular}{@{}l|cc|ccc@{}}
% \hline
% % Image     & b& P  & \multicolumn{7}{c}{SNR}  \\
% % \cline{4-11}
% &Train Frame      &Test Frame& MVBench&MuitiClip \\
% \hline
% B1&8  &8   &     46.0 &53.2 \\
% B2&8  &16   &   46.7  & 54.8\\

% \hline
% B3&16  &16   &48.3      &57.0 \\
% B4&16  &32   &48.6      & 57.6\\
% B5&16  &4z8   &48.8      & 58.8\\
% \hline
% \end{tabular}
% }
% \caption{Results of different setting of training frames and inference frames.}\label{tab:9}
% \end{table}


==> ICCV2025-Author-Kit-Feb/sec/conclusion.tex <==
\section{Conclusion}

% We propose a visual compression module that significantly reduces the number of tokens, thereby substantially lowering computational costs of training and inference for large language models (LLMs), while maintaining or even improving model performance. Additionally, to address the issue of data scarcity in multi-camera scenarios, we develop an automated video annotation pipeline to label datasets, enhancing model capabilities in real-world multi-scene applications. Furthermore, we construct a specialized test set to evaluate model performance in these scenarios.
% To address the multi-shot video understanding problem, we propose proprietary datasets and a novel model. We tackle data scarcity in multi-camera scenarios by developing an automated video annotation pipeline to generate both training and testing datasets. Furthermore, we introduce an instance-based visual compression module for multi-scene challenges. Our dataset and model significantly enhance multi-scene video understanding and show unique advantages across various video benchmarks.............
% However, the pre-trained model used in our approach is not based on the latest foundational model. We will continue to explore the compatibility of our model with better foundational models to further enhance its performance.


Recognizing a gap not previously addressed in the handling of multi-shot videos with VideoLLMs, we identify the deficiencies and their underlying causes. This lead us to propose proprietary datasets and a novel design. By developing an automated video annotation pipeline, we tackle data scarcity in multi-shot scenarios. Furthermore, we introduce an instance-based visual compression module for multi-scene challenges. Our dataset and model significantly enhance multi-scene video understanding and demonstrate unique advantages across various video benchmarks.


==> sec/1_intro0.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.95\linewidth]{pic/F1_last.pdf}
\caption{\textbf{Multi-shot Transitions} Video-LLaVA uses full projection, while 
 VideoChat1/2 reduce video tokens using attention mechanisms. In scenes with discontinuous character appearances (multi-scene transitions), existing models often struggle to distinguish characters, causing counting errors. Ours compresses tokens and uses detectors and clustering as instance prompts to guide attention information mixing, improving accuracy.
}	\label{fig:1}
\vspace{-13pt}
\end{figure}

\section{Introduction}
%The development of large language models (LLMs) [] has paved the way for Multi-modal Large Language Models (MLLMs) [],  and the integration of visual encoders with pre-trained LLMs to form visual multi-modal large models [] has gained significant research attention. 
The  Multi-modal Large Language Models (MLLMs) ~\cite{alayrac2022flamingo,driess2023palm,huang2023language,li2023blip,li2023videochat,liu2023visual,wang2024qwen2,zhu2023minigpt} attract significant attention. Among these, 
% video large models
video LLMs~\cite{lin2023video,li2024mvbench,zhang2023video,xu2024pllava,team2024gemini} face numerous challenges, such as long video understanding~\cite{liu2024st,song2024moviechat}, fine-grained understanding~\cite{wang2022internvideo,li2024llava}, and temporal localization~\cite{chen2024timemarker,wang2024grounded,patraucean2023perception,li2023seed}. To meet the demands of these specific tasks,  various video benchmarks and model designs have emerged, demonstrating remarkable capabilities. . %The advent of LLMs has significantly improved the ability to automatically annotate video questions ~\cite{maaz2024videogpt+,li2024mvbench},  and a common practice now is to generate question-answer pairs from detailed video descriptions or captions. 
We find that, despite the existence of many benchmarks~\cite{li2024mvbench,fu2024video,caba2015activitynet,xiao2021next,lei2018tvqa,mangalam2023egoschema,yi2019clevrer} for evaluating video models, they still struggle to effectively reflect the performance in common real-world scenarios, such as multi-shot videos with multiple scene transitions.

\wzc{The Multi-modal Large Language Models (MLLMs) have yielded remarkable results. Regarding video data, there has been a significant emergence of Video LLMs dedicated to long video understanding and fine-grained understanding, which have demonstrated remarkable capability. However, we observe that although current video LLMs have demonstrated robust capabilities in video understanding, they exhibit notable deficiencies in multi-scene videos. }

\wzc{Videos containing multiple distinct scenes are formally termed multi-scene video. Compared to single-scene video, such compositions require enhanced temporal segmentation capacity and instance-level comprehension, thereby enabling robust understanding of dynamic transformations and relational dependencies among instances across scenes. As shown in Fig~\ref{fig:1}, previous video LLMs struggle with the question related to multi-shot scenes. Through investigation of this phenomenon, we show that such issue stems from the scarcity of training data tailored to multi-scenes and architectural limitations in prevailing model frameworks. From a data perspective, while existing video datasets demonstrate quantitative abundance, their compositional emphasis predominantly lies in single-scene, with high-dynamic multi-scenes videos constituting merely marginal proportions. Furthermore, current QA formulations inadequately meet multi-scenes understanding requirements. Current QAs are more for the understanding of the whole video and not for the understanding of the different scene levels. Moreover, current widely used benchmark can hardly reflect the ability for multi-scene video understanding because of the lack of consideration of multi-scene, an important video type, in its design. Therefore, it is essential to propose a tailored training set and benchmark for multi-scene video understanding.}

\wzc{To address the gap in multi-scenario benchmarks, we propose a multimodal video understanding benchmark called \textbf{MultiClip-Bench}. Compared to existing benchmarks\cite{wang2023internvid,krishna2017dense,maaz2024videogpt+,li2024mvbench,mangalam2023egoschema,fu2024video}, our dataset stands out in its annotation format and question design. %First, we introduce an automatic selection and annotation pipeline to create the dataset. 
 Ours video descriptions are built on three key elements: keyframe annotations with character IDs, dense captions, and character information annotations, all aimed at covering multi-scene understanding. We segment the video into keyframes and annotate each keyframe sequence with character IDs to ensure correct association of individuals across scenes, maintaining character consistency.  Based on this, we generate dense captions and character information annotations for video, which also connect fragmented scenes involving the same person. We then focus on scenarios where characters appear discontinuously across multiple scenes or have brief appearances (time criteria are used only for dataset generation). These efforts address potential issues in multi-shot scenes and generate question-answer pairs to enhance instruction-following capabilities. From these, we manually selected a subset of $2,750$ pairs to form the test set, with answers verified, refined, and categorized to create the Benchmark.}

 \wzc{Thanks to the benchmark we proposed, we found that existing models perform poorly in handling multi-shot videos. To obtain the ideal model satisfying video LLM,
we identify several requirements for obtaining satisfying video LLM: 
% in the process of obtaining the CAD features, 
(a) efficient processing of large numbers of video frames to preserve key frame information between scene transitions; 
% Second, 
(b) ability to capture information about instances in different scenarios, thus improve cross-scene understanding ability.
Unfortunately, current video LLMs do not satisfy both conditions and tend to ignore the important instance information in multi-scene video. Motivated by the requirements, we propose a new model named \textbf{IPformer-VideoLLM}, which uses \textbf{instance prompts} to guide attention for better instances feature aggregation. Specifically, we sample and aggregate features from bounding box regions into instance features, injecting them as visual prompts into the query to guide attention. This reduces tokens to under 10\% of the baseline, cuts training time by 75\%, and boosts inference speed. Experiments show strong performance on our benchmark and others, ith further performance improvements achieved when trained on our proposed dataset.
}

Multi-shot videos often present challenges in understanding fragmented scenes. For instance, when multiple people appear in discontinuous scenes, the question "How many people in the video?" (as shown in Fig ~\ref{fig:1}). Such questions, which involve multi-scene transitions, have not been adequately addressed or summarized by existing benchmarks. The main cause lies in the lack of high-quality annotations tailored for multi-scene understanding.  Current video descriptions typically\cite{wang2023internvid,krishna2017dense,maaz2024videogpt+,luo2023valley} provide a general summary of the entire video, focusing on  key actions of key 
 individuals, striking content, or the overall atmosphere. However, this annotations is not suitable for multi-shot scenarios. The core challenge lies in how to separate unrelated scenes and connect multiple related yet discrete shots, which should be considered related. For instance, in Fig.~\ref{fig:1}), the female judge appears in only one frame, which should be treated as an independent scene. Meanwhile, the male judge appears in frames 1, 2, and 8. However, current video annotations often focus solely on describing the key actions or appearance of the man, neglecting his association across different shots, and even entirely omitting any mention of the female judge. Can such annotations help the model recognize that the man at the beginning and end is the same person? Will less prominent scenes, like those with the female judge, be ignored? Moreover, question-answer pairs from these inadequate annotations fail to address the core challenges of multi-scene understanding.

 To address the gap in multi-scenario benchmarks, we propose a multimodal video understanding benchmark called \textbf{MultiClip-Bench}. Compared to existing benchmarks\cite{wang2023internvid,krishna2017dense,maaz2024videogpt+,li2024mvbench,mangalam2023egoschema,fu2024video}, our dataset stands out in its annotation format and question design. %First, we introduce an automatic selection and annotation pipeline to create the dataset. 
 Ours video descriptions are built on three key elements: keyframe annotations with character IDs, dense captions, and character information annotations, all aimed at covering multi-scene understanding. We segment the video into keyframes and annotate each keyframe sequence with character IDs to ensure correct association of individuals across scenes, maintaining character consistency.  Based on this, we generate dense captions and character information annotations for video, which also connect fragmented scenes involving the same person. We then focus on scenarios where characters appear discontinuously across multiple scenes or have brief appearances (time criteria are used only for dataset generation). These efforts address potential issues in multi-shot scenes and generate question-answer pairs to enhance instruction-following capabilities. From these, we manually selected a subset of $2,750$ pairs to form the test set, with answers verified, refined, and categorized to create the Benchmark.

 Through the benchmark we proposed, we found that existing models perform poorly in handling multi-shot videos. These models rely on full projection of visual tokens\cite{lin2023video,li2024llava,xu2024pllava,wang2024qwen2}, to achieve good results, but they are slow and support only a limited number of frames, making efficient token compression a key challenge\cite{bai2023qwen,zhang2025llava,zhang2023video,song2024moviechat,ye2024mplug,liu2024st}. For example, Qformer\cite{li2023blip} mixes frame features using learnable query tokens but faces high training difficulty. Hence our first goal is to design a more efficient compression method to accommodate more frames; Existing models split highly correlated regions into independent tokens, fragmenting instances features. Our second goal is to aggregate these features across scenes. To address this, we propose \textbf{IPformer-videoLLM}, which uses \textbf{instance prompts} to guide attention for better  instances feature aggregation. Specifically, we sample and aggregate features from bounding box regions into instance features, injecting them as visual prompts into the query to guide attention. This reduces tokens to under 10\% of the baseline, cuts training time by 75\%, and boosts inference speed. Experiments show strong performance on our benchmark and others, ith further performance improvements achieved when trained on our proposed dataset.
% The development of large language models (LLMs) has laid the foundation for Multi-modal Large Language Mod
% els (MLLMs), with vision-centric models (e.g., GPT-4o, LLaVA, InternVL series) enabling LLMs to understand visual information such as images and videos. The mainstream approach involves encoding images or video sequences and flattening them then aligning them to the textual space via linear projection[]. However, in practical applications, as shown in Figures ~~\ref{{fig:1}} and ~~\ref{fig:PLLava}, tokenization based on fixed-size patches performs poorly in scenarios involving instance consistency understanding and shot transitions. This may be attributed to: (1) conflicts between language models and visual tokenization, where fixed-size tokenization splits correlated regions into independent tokens, leading to issues like individual truncation and overlooked small objects; and (2) insufficient frame sampling, where limited frames (e.g., 8 frames) fail to capture sufficient visual information in complex scenes. To address these challenges, current models[] adopt higher-resolution images and more frames, significantly increasing computational costs, making efficient video token compression a key focus Among the compression schemes, the attention-based approach achieves a higher compression rate compared to methods like average pooling (avg-pooling), significantly reducing the number of tokens. However, the attention module converges more slowly and typically requires more complex training procedures [] and larger amounts of data [] to effectively learn the attention mechanism and the learnable query. Moreover, its performance often falls short of methods like average pooling. One of our goals is to optimize the attention-based approach so that it can achieve better performance than uncompressed methods (full projection) under the same amount of data.

%语言大模型（LLM）的发展为多模态大模型（LMMs）奠定了基础，其中视觉大模型（如GPT-4o、LLaVA、InternVL系列）赋予了LLM对图像和视频等视觉信息的理解能力。目前主流方法通过Vision Transformer（ViT）将图片或视频序列编码后展平，并利用线性投影将其对齐到文本空间[]。然而，在实际应用场景中，如图1和图2所示，基于等大小token化的方案在处理实例不连续或镜头切换的场景时表现不佳。这可能源于以下原因：1.语言模型与视觉token化的特性冲突：语言模型中单词间具有离散性，而图像等大小token化会将强相关区域分割为独立token，导致人物截断等问题，不利于后续推理。小人物等重要细节容易被忽略，进一步影响模型性能。2.视频帧采样不足：当前模型通常仅使用有限帧数（如8帧），难以提供足够的视觉信息，尤其在复杂场景中可能导致关键信息丢失。为了提升效果，当前模型[]倾向于采用更高分辨率的图像和更多的视频帧数，但这显著增加了计算成本，使得视频信息压缩成为研究重点。现有视频压缩方法多样（详见Related Work）。其中基于注意力机制的压缩方案相较于基于平均池化（avg-pooling）等方法，其压缩率更大，能显著减少token数量，然而这个attention模块收敛慢，他们通常需要更复杂的训练流程[]和更多数据[]去更好学习attenion模块和可学习的query，且效果也不如平均池化等方法。我们的目标之一是优化基于attenion的方案，使其在同样数据的情况下达到相比于不压缩（全投影）更好的性能。

% 1. 因为需要更多的信息，所以需要更多的视觉token，但是如果直接使用的话，对于视觉token当中的冗余性就太强了，从而导致性能虽然提升，但是不值得。2. 因此需要token compression的方式，保存更多有效的token，去除冗余的token。3. 两种基本方式，对于视频而言，因为其对于帧率和分辨率的要求，所以需要更高的压缩率。目前基于attention的压缩方式的压缩率高，但是存在有性能和训练的问题，因此我们的模型的目的就是解决这个问题。提升压缩率，同时有更好的性能和训练收敛。

% 我认为模型这边的说法，需要和multi-shot scenes结合一下。

% 在多场景的视频数据环境下，存在的问题。1. 视频数据需要压缩，从而才可以有更好的理解能力。2. 目前的压缩方法，对于多场景的视频数据效果不佳：因为目前很多压缩是pooling这类的方式，可能会将不属于同一个场景的压缩到一起（一般可能直接的类似于pooling的压缩方式会存在有将不同场景直接合并的问题），但是动态的压缩方式，比如attention的方式，目前的性能和训练时存在明显的问题。这样才能支持存在多场景的视频数据的压缩要求。
% 因此从我们的任务的需求出发， 我们需要开发一个易于训练的，性能好的，动态压缩方式（基于attention）

% The development of video understanding is somewhat constrained by the low quality of video-text data. Existing research [] explores various aspects such as high video quality, video localization, and timestamps. Relevant to our work, ....[] points out that existing video-text datasets lack dynamism, with much of the content being describable by a single image, lacking the temporal understanding challenges unique to video scenarios. In contrast, we focus on the comprehension difficulties caused by multi-shot transitions in videos, such as person re-identification, as shown in Figure ~re. This task requires recognizing the same individual across discontinuous appearances, demanding an understanding of continuity. Previous models and datasets have rarely addressed this scenario, and there is a lack of relevant datasets. 

% 还需要把模型和数据集串起来，可能会更好一些。

%视频理解的发展一定程度受制于视频-文本数据的低质量。现有研究[]从不同的角度研究高视频质量，视频定位，时间戳等方向。其中与我们相关的是,...提出[]现有的视频-文本数据集的动态性差，很多内容是一张图片就能描述的，不具有视频场景下独有的时序理解等困难。而我们专注于视频多镜头切换带来的理解困难，比如行人重识别，如图1所示，要求要能识别不连续出现的人是同一个人，这要求具有理解连贯性。之前的模型和数据很少研究此场景，缺乏相关的数据集。  

% 目前视频理解的难点在于对多场景下的理解，这个其中的一个核心原因是在于目前对于多场景数据集的工作的缺失。 之前的工作xxx。因此我们提出这个数据集对于提升多场景理解，从而提升对于视频理解的能力是必要的。

% In this paper, our research objectives are twofold: (iTo explore a more efficient video visual token compression framework that uses fewer tokens to achieve faster and more efficient visual information processing in multi-shot and other complex scenarios, while maintaining or even improving model performance. (ii To construct a dedicated multi-shot scene dataset, as we found that current research on multi-shot scene understanding lacks specialized datasets, which may severely limit the model's ability to comprehend such scenarios.

% 在本文中，我们的研究目标是提升模型对于多场景的视频数据的理解能力。其中具体的可以分为两个方面，1. 从模型结构上，设计了一个模型视觉token压缩器，有利于提升模型对于包含多场景的视频的理解能力。2. 提升了相关的数据集。

%在本文中，我们的研究目标分为两个方面：1.探索更高效的视频视觉token压缩框架采用更少的toke在多镜头场景及其他复杂场景中实现更快、更高效的视觉信息处理，同时保持或提升模型性能。2.构建多镜头场景相关数据集：我们发现，当前关于多镜头场景理解的研究缺乏专门的数据集，这可能严重限制模型在该场景下的理解能力。

% For the first objective, we propose a compression framework based on cross-attention, drawing inspiration from Conditional-DETR and improving learned queries. Specifically: 1.Injecting frame-level information to enhance token order: We sequentially inject the cls-token and global-avg-token of each frame into each query token, providing guidance for subsequent information mixing and preserving token order. 2.External detector for instance supplementation: To address the lack of instance information, we introduce an external detector to identify all potential instances. Features corresponding to each detected bounding box are sampled and aggregated, then injected into the query tokens. This operation is similar to the anchor mechanism in object detection[], guiding the query tokens in their interaction with subsequent video sequence features. Under the same experimental setup[], we reduce tokens from 8×256 to 8×20, achieving a Speedup is approximately 3 times (excluding the external detector). inference speedup and a 1.1 point performance gain on dataset[].


% For the second objective, we constructed a dataset specifically designed for multi-shot scenes, consisting of two parts: Training set: We propose an automatic selection and annotation pipeline to create the dataset, which includes keyframe annotations, dense captions, and character information annotations to improve the quality of multi-shot scene labeling. We focus on scenarios with discontinuous characters across multiple scenes, identifying potential issues in multi-shot scenes and generating QA pairs to enhance instruction-following capabilities. Test set: From the generated QA pairs, we manually select a subset as the test set, where answers are verified, refined, and categorized to form the final evaluation set. We tested our model and other models on this dataset, demonstrating that our model and training set effectively improve the understanding of multi-shot scenes.
%针对第一点，我们提出了一种基于cross-attenion的压缩框架，并参考了Conditional DETR的设计，对learned query进行了改进。具体方法如下：1.注入帧级信息以增强token顺序性：将每帧的cls-token和global-avg-token按顺序注入到每个query token中，为后续的信息混合提供引导，从而保留token排列的顺序性。为了弥补实例信息的缺失。2.外接检测器以补充实例信息：为了弥补实例信息的缺失，我们引入了一个外部检测器，用于检测潜在的所有实例。通过对每个检测框（box）所在区域的特征进行采样和聚合，将这些实例特征注入到query token中。上述操作与目标检测中的给定anchor机制类似，能引导其query token和之后视频序列的特征混合。针对第二点，我们构建了一个专门面向多镜头场景的数据集，包括以下两部分：训练集：我们提出了自动选择和标注的流程来制作数据集，其内容包含关键帧标注，密集字幕，和人物信息标注来提高多镜头场景标注的质量。我们多场景下不连续人物的场景，挖掘多镜头场景中可能存在的问题，生成QA对，提高指令遵循能力。测试集：对生成的QA对，我们人工选择一部分作为测试集，对答案进行饺子且分类，形成测试集，我在我们的模型和其他模型进行测试，表面我们的模型和训练集能有效提高这个多镜头场景的理解能力。


% 除此以外，也在更广泛的视频benchmark上测试了性能，验证了这个问题是视频理解中广泛存在的。

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
